Planning for Package Deliveries in Risky Environments Over Multiple Epochs

We study a risk-aware robot planning problem where a dispatcher must construct a package delivery plan that maximizes the expected reward for a robot delivering packages across multiple epochs. Each package has an associated reward for delivery and a risk of failure. If the robot fails while delivering a package, no future packages can be delivered and the cost of replacing the robot is incurred. The package delivery plan takes place over the course of either a finite or an infinite number of epochs, denoted as the finite horizon problem and infinite horizon problem, respectively. The dispatcher has to weigh the risk and reward of delivering packages during any given epoch against the potential loss of any future epoch's reward. By using the ratio between a package's reward and its risk of failure, we prove an optimal, greedy solution to both the infinite and finite horizon problems. The finite horizon problem can be solved optimally in $O(K n\log n)$ time where $K$ is the number of epochs and $n$ is the number of packages. We show an isomorphism between the infinite horizon problem and Markov Decision Processes to prove an optimal $O(n)$ time algorithm for the infinite horizon problem.

==> algorithms.tex <==
\section{Algorithms}

In this section, we provide greedy algorithms to solve RTPD, and RSPD. For RTPD we show an exponentially decaying approximation factor while for RSPD we show an optimal, linear time solution.





==> general_problem_formulation.tex <==

\section{Problem Formulation}
Consider a set of tasks $\mathcal{T} = \{t_1, t_2, ..., t_n\}$ where each task, $t_i \in \mathcal{T}$, has an associated reward, $r_i \in \mathbb{R}_{+}$. A team of $\alpha$, homogeneous agents are allocated at the beginning of a $k$-day mission to accomplish the tasks in $\mathcal{T}$. Before the mission begins, a subset of tasks is chosen for each day, i.e., $T = \{T_h \subseteq \mathcal{T} : \forall h \leq k  \}$, and the agents are restricted to only those tasks on that day. On any given day, each agent follows a walk, i.e., an ordered sequence of tasks $W = \{ t_{w,1}, ..., t_{w,\mu} \}$, through the days subset of tasks to collect rewards. After the reward from a task is given, the task cannot be accomplished again on the same day by any agent. $T$ is known to the agents before the mission begins so they can plan their walks beforehand. On each day, all agents begin their first walk at a "rest" task, $t_0$, which does not give a reward. Each agent is restricted to accomplishing only $\mu$ tasks in a row before they must return to their rest task. The agents can always take the rest task early, though for some scenarios this may not be advantageous. This restriction on the number of tasks in a row means that we can break up every agents walk into a sequence of tasks that begins and ends on the same task, i.e. a set of closed walks, $C(W) = \{ W_1, W_2, ..., W_p \}$, each beginning and ending on $t_0$.

Additionally, while the agents are following their walks, there will be a risk of failure between each pair of tasks. If an agent fails between two tasks, a cost of $\theta$ is incurred and the agent cannot accomplish any future tasks. Let $\rho({i,j}) \in [0,1]$ be the probability an agent can successfully accomplish task $t_j$ given it just finished accomplishing task $t_i$. The probabilities are symmetric, i.e. $\rho({i,j}) = \rho({j,i})$, and their logarithms also satisfy the triangle inequality, i.e., $\log \rho({i,j}) + \log \rho({j,k}) < \log \rho({i,k})$, which is equivalent to $\rho({i,j})\rho({j,k}) < \rho({i,k})$. This means we do not consider tasks which can proactively improve the likelihood of success for other tasks. Given any closed walk $W_i \in C(W)$, let $\psi_{i}$ be the probability of accomplishing all tasks in $W_i = \{ t_0, t_{i,1}, ..., t_{i_{\mu,i}}, t_0 \}$, including the previous and last rest task. Let $\mu_i \leq \mu$ be the number of tasks in $W_i$. The probability of finishing $W_i$ should depend on the probability of finishing every previous closed walk. Then, the probability of finishing $W_i$ is calculated by:

 \begin{equation}
     \psi_i = \psi_{{i-1}}\prod_{j < \mu}{ \rho({t_{i,j},t_{{i,j+1}}})}
 \end{equation}
 
 Assume for the base case calculation of $\psi_1$ that $\psi_{{0}} = 1$. Naturally, the probability that any agent fails on any given day is equal to the probability it does not finish its last closed walk, i.e. $(1 - \psi_p)$.
 The goal of the team of agents is to maximize the expected reward in a mission despite the risk of failure along their walks.

To begin, we will provide the expected reward for a single agent assigned a set of walks through $\mathcal{T}$ for a single day mission. Given any closed walk, $W_i$, we denote $r_{i,m}$ to be the reward of task $t_{i,m} \in W_i$ and $\psi_{i,m}$ to be the probability of receiving reward $r_{i,m}$.  We make the distinction that for some scenarios, the probability of receiving a reward from a task is not necessarily equal to the probability of accomplishing the task. One example of such a scenario is where an agent must collect packages and then drop them off at a depot. The probability that an agent collects a package is not equal to the probability of the agent dropping off the package, i.e., the depot earning its reward for a retrieved package. Here, we abstract $\psi_{i,m}$ to its most general form, irrespective of any scenario. Then, the expected reward for a team of one agent to accomplish its set of ordered walks for a single day mission is: 

\begin{equation}
    \bar{E}(\mathcal{C}) = \sum_{W_i \in C(W)}\sum_{m=0}^{\mu_i}r_{i,m}\psi_{i,m} - \theta (1 - \psi_p) \label{eq_singleagent_relativised_expectation}
\end{equation}

From here, we can better see the expected reward for a team of agents on a single day. Namely, let $\mathcal{C} = \{ C_1, \ldots, C_\alpha \}$ be the set of closed walks for each agent on a given day. Let $P(\beta | \alpha)$ be the conditional probability of $\beta$ agents finishing the day if $\alpha$ agents were allocated at the start. $P(\beta | \alpha)$ can be calculated by taking the probability of finishing the day for each agent as a trial in a Poisson Binomial distribution. Then, $P(\beta | \alpha)$ is the probability of $\beta$ successful trials[Reference]. So, the expected reward for a team of $\alpha$ agents to accomplish their set of ordered walks for a single day mission is given by:

\begin{equation}
    \bar{E}(\mathcal{C}) = \sum_{C_j \in \mathcal{C}}\sum_{W_i \in C_j}\sum_{m=0}^{\mu_i}r_{i,m}\psi_{i,m} - \theta\sum_{\beta = 0}^\alpha P(\beta | \alpha)(\alpha - \beta) \label{eq_multiagent_relativised_expectation}
\end{equation}

One can easily verify that \ref{eq_multiagent_relativised_expectation} reduces to \ref{eq_singleagent_relativised_expectation} if $\alpha = 1$. Finally, we will expand the expectation for missions involving multiple days. Let $E(\mathcal{C}_h)$ be the expected reward on day $h$ given a collection of closed walks for day $h$, $\mathcal{C}_h$, if $\alpha$ agents are allocated on day 1. The definition of $\mathcal{C}_h$ has to be expanded to a collection of sets of closed walks, $\mathcal{C}_h = \{\mathcal{C}_{h,1}, \ldots, \mathcal{C}_{h,\alpha}\}$. If only $\beta$ agents survive to day $h$, then changing the assigned closed walks to $\mathcal{C}_{h,\beta}$ is required to accommodate the lost agents. Due to the linearity of expectation, the most general form of our problem is the following:

\begin{problem}
 Risk-Aware Multi-Agent Heterogeneous Planning (RAMAHP)
\end{problem}
 \begin{equation}
    \text{Find   } \text{arg}\max_{\mathcal{C}_1,\ldots,\mathcal{C}_k} \sum_{h \leq k} E_h(\mathcal{C}_h)
    \label{eq:RMAHP}
\end{equation}

Let $P_{h-1}(\beta | \alpha)$ be the probability of having $\beta$ agents survive day $h - 1$ given $\alpha$ were allocated to the mission. Then, the following proposition follows naturally from conditional probability.

\begin{proposition}
    \begin{equation}
        E_h(\mathcal{C}_h) = \sum_{\beta \leq \alpha}P_{h-1}(\beta | \alpha) \bar{E}(\mathcal{C}_{h,\beta})
        \label{eq:expectation_day_h}
    \end{equation}
    \label{prop:expectation_day_h}
\end{proposition}
\begin{proof}
To find the total expectation, one must sum over all possible events for a day. In this case, we must sum over all possible rewards and all possible ways of incurring a cost.
$E_h(\mathcal{C}_h)$ is defined explicitly as:
\begin{align*}
        E_h(\mathcal{C}_h) &= \\ &\sum_{\beta \leq \alpha} \sum_{C_j \in \mathcal{C}_{h,\beta}}\sum_{W_i \in C_j}\sum_{m=0}^{\mu_i}r_{i,m}\psi_{i,m}P_h(\beta) \\ &- \sum_{\beta \leq \alpha}\theta\sum_{\beta' \leq \beta} P_h(\beta' | \beta)P_h(\beta)(\beta - \beta')        
\end{align*}
Where $P_h(\beta)$ is the probability of having $\beta$ agents at the start of day $h$, which is equivalent to $P_{h-1}(\beta|\alpha)$ Then, by pulling out $P_h(\beta)$ one obtains the proposition.
\end{proof}

By the law of total probability, we can define $P_{h-1}(\beta|\alpha)$ from Proposition \ref{prop:expectation_day_h} more explicitly:
\begin{definition}[Probability of Agents Surviving to a Given Day]
\begin{equation}
    P_{h-1}(\beta|\alpha) = \sum_{\beta \leq \beta_{2} \ldots \leq \beta_1} P_{h-1}(\beta | \beta_{2})P_{h-2}(\beta_{2}|\beta_{3}) \ldots P_1(\beta_1|\alpha)
    \label{eq:prob_survival_to_day}
\end{equation}
\label{def:prob_survival_to_day}
\end{definition}

Substituting (\ref{eq:prob_survival_to_day}) and (\ref{eq:expectation_day_h}) into (\ref{eq:RMAHP}) reveals a dynamic programming solution. Let $V_h(\beta)$ be the expected reward for all remaining days if only $\beta$ agents survive to day $h$. 

\begin{definition}[Bellman Equation for RAMAHP]
\begin{equation}
    V_h(\beta) = \max_{\mathcal{C}_{h,\beta}} \bar{E}(\mathcal{C}_{h,\beta}) + \sum_{\beta' \leq \beta}P_h(\beta'|\beta) V_{h+1}(\beta')
    \label{eq:Bellman_eq}
\end{equation}

\begin{equation}
    V_k(\beta) = \max_{\mathcal{C}_{k,\beta}} \bar{E}(\mathcal{C}_{k,\beta})
    \label{eq:Bellman_eq_base}
\end{equation}
\label{def:bellman_eq_RAMAHP}
\end{definition}
\begin{proof}
We will prove this definition by induction. Naturally, the base case, \ref{eq:Bellman_eq_base}, is true by definition. Assume that we have calculated the optimal closed walks to maximize the expected reward for days $i + 1$ to $k$ for all number of available agents on day $i + 1$. Then, $V_{i + 1}(\beta')$ is optimal for all $\beta' \leq \beta$. Using definition 
\end{proof} 

For the sake of intuition, we will restrict ourselves to a package delivery scenario. simplicity, we will assume that the reward for all tasks in a closed walk are given before the beginning of the next closed walk, i.e. $\psi_{i,m} < \psi_{j,m'}$ for any $t_{i,m}$ and $t_{j,m'}$ if $i < j$.

Each agent's goal is to maximize the overall expected reward across all days by accomplishing as many tasks as possible before failure.

There are two alternative scenarios we consider for when a reward is given. Either the rewards are given upon accomplishing a task, i.e. a package delivery scenario, or they are given during the rest state, i.e. a package collection scenario. The expected reward for each scenario is similar. The properties we prove in this work do not rely on either scenario, however the package delivery scenario maintains the general form. In fact, the package collection scenario can be seen as a restriction on the package delivery scenario by assigning the probability of receiving a task to be the same as the probability of completing the cycle.

\subsection{Package Delivery Scenario}
Impose a maximum number of tasks an agent can accomplish before resting to obtain more packages by an upper limit on the cycles, $\mu_\text{max}$.
\begin{equation}
    E(C(W)) = \sum_{i=1}^p\sum_{m=0}^{\mu_\text{max}}r_{i,m}\psi_{i,m}-\theta(1-\psi_p)
\end{equation}

\subsection{Package Collection Scenario}
By imposing $\forall m \leq \mu_i : \psi_{i,m} = \psi_{i}$, then $\sum_{m=0}^{\mu_i}r_{i,m}\psi_{i,m} = R_i\psi_i$ where $R_i = \sum_{m=0}^{\mu_i}r_{i,m}$.
\begin{equation}
    E(C(W)) = \sum_{i=1}^p R_{i}\psi_{i}-\theta(1-\psi_p)
\end{equation}
This scenario is equivalent to the problem presented in \cite{PRASAD2019321}.

\begin{problem}
 Single-Agent Risk-Aware Task Execution (SARATE)
\end{problem}

\begin{equation}
    \text{Find   } W* \in \text{arg}\max_{W \in \mathcal{W}} E(C(W))
\end{equation}

\section{Characteristics of Optimal Walks}

This section proves some characteristics about optimal walks for the SARATE problem. Many of these properties carry over from previous work by \cite{PRASAD2019321}, however they are crucial and worth restating for this general case. In fact, the first property we will prove is that this formulation of the SARATE problem is isomorphic to the metric space version in \cite{PRASAD2019321}. Rather than considering probabilities between tasks, we consider distances between tasks. 

\begin{proposition}
Consider a weighted graph, $G = (V,E)$, where $V = T \cup \{t_0\}$ and $E = \{ (t_u, t_v) : t_u, t_v \in V, t_u \ne t_v \}$.  Each edge $e = (t_u,t_v) \in E$ has a weight $w(e) = w(t_u,t_v)$ denoting the distance between tasks $t_u$ and $t_v$. Let each triplet of edges in $E$ satisfy the triangle inequality. Define $\phi$ to be the probability of success per unit distance of the agent.
\end{proposition}

 Then, the probability the agent is able to travel from $t_u$ to $t_v$ is $\phi^{w(t_u,t_v)}$. More generally, the probability of traversing a walk is $\phi^{d}$ where $d$ is the total distance of the walk. Using this notation, we can map our version of SARATE to the metric space version.

\begin{align*}
    \max_{C\in \mathcal{C}}E(C(W)) = \max_{C\in \mathcal{C}} \sum_{i = 0}^{p} \sum_{m = 0}^{\mu_i} r_{i,m} \psi_{i,m} - \theta(1 - \psi_p)
\end{align*}

\begin{align*}
    \max_{W\in \mathcal{W}}E(W) = \max_{W\in \mathcal{W}} \sum_{i = 0}^{p} \sum_{m = 0}^{\mu_i} & r_{i,m} \phi^{\log_\phi \psi_{i,m}} \\ & - \theta(1 - \phi^{\log_\phi{\psi_p}})
\end{align*}

\begin{align*}
    \log_\phi{\psi_{i,m}} & = \log_\phi { \prod_{j \leq i, m < \mu_j} \rho(W_{j,m}, W_{j, m+1}) } \\ & = \sum_{j \leq i, m < \mu_j} \log_\phi{\rho(W_{j,m}, W_{j, m+1})}
\end{align*}

By defining $d_{i,j} = -\log_\phi \rho(i,j)$ and $d_k = -\log_\phi{\bar{\phi}_k}$, then $d_{i,j}$ can be interpreted as the distance between tasks $i$ and $j$, i.e., $w({i,j})$, and $d_k$ is the total distance of cycle $k$. Then, $\phi$ is the probability of failure per unit distance.

\begin{align*}
    \max_{W\in \mathcal{W}}E(W) = \max_{W\in \mathcal{W}} \sum_{i = 0}^{p} \sum_{m = 0}^{\mu_i} & r_{i,m} \phi^{\sum_{k=1}^{i-1}d_k}\phi^{\sum_{j=1}^m d_{i,j}} \\ & - \theta(1 - \phi^{d_p})
\end{align*}

Inverting this process to show an isomorphism is straightforward from the other direction as well. Construct a distance between tasks such that $\phi^{w(t_u,t_v)} = \rho(t_u,t_v)$. Because $\log \rho(t_u,t_v)$ satisfies the triangle inequality, the edges in $G$ also satisfies the triangle inequality for every triplet of tasks in $T$. 

Because the two problems are isomorphic, their optimal solutions are also isomorphic.

\subsection{Reward-to-Risk Ratio}



\begin{equation}
    \gamma_i = \frac{\sum_{m=0}^{\mu_i} r_{i,m}\psi_{i,m} }{1 - \psi_i}
\end{equation}

\subsection{Ordering of Cycles by Reward to Risk Ratio}


\begin{align*}
    \frac{\sum_{m=0}^{\mu_i} r_{i,m} \bar{\psi}_{i,m} }{1 - \bar{\psi}_i} < \frac{\sum_{m=0}^{\mu_{i+1}} r_{i+1,m} \bar{\psi}_{i+1,m} }{1 - \bar{\psi}_{i+1}}
\end{align*}
 


\begin{align*}
    \rightarrow &(\sum_{m=0}^{\mu_i} r_{i,m} \bar{\psi}_{i,m}) +   \bar{\psi}_i(\sum_{m=0}^{\mu_{i+1}} r_{i+1,m} \bar{\psi}_{i+1,m}) \\ &<   (\sum_{m=0}^{\mu_i} r_{i,m} \bar{\psi}_{i,m}) + \bar{\psi}_{i+1}(\sum_{m=0}^{\mu_i} r_{i,m} \bar{\psi}_{i,m}) \label{eq:}
\end{align*}
 


Let $\bar{W}$ be the same as $W^*$ except with $W_i$ and $W_{i+1}$ swapped. $E(\bar{W}) - E(W^{*})$



\begin{align*}
    &E(\bar{W}) - E(W^{*}) = \\& (\sum_{m=0}^{\mu_{i+1}}r_{i+1,m}\bar{\psi}_{i+1,m})\prod_{k=0}^{i-1}\bar{\psi}_k + \bar{\psi}_{i+1}(\sum_{m=0}^{\mu_i}r_{i,m}\bar{\psi}_{i,m})\prod_{k=0}^{i-1}\bar{\psi}_k \\&- (\sum_{m=0}^{\mu_i}r_{i,m}\bar{\psi}_{i,m})\prod_{k=0}^{i-1}\bar{\psi}_k - (\sum_{m=0}^{\mu_{i+1}}r_{i+1,m}\bar{\psi}_{i+1,m})\prod_{k=0}^{i}\bar{\psi}_k
\end{align*}

\begin{align*}
    = &(\sum_{m=0}^{\mu_{i+1}}r_{i+1,m}\bar{\psi}_{i+1,m}) + \bar{\psi}_{i+1}(\sum_{m=0}^{\mu_i}r_{i,m}\bar{\psi}_{i,m})\\ &- (\sum_{m=0}^{\mu_i}r_{i,m}\bar{\psi}_{i,m}) - \bar{\psi}_{i}(\sum_{m=0}^{\mu_{i+1}}r_{i+1,m}\bar{\psi}_{i+1,m})
\end{align*}
    

By the previous slide, $E(\bar{W}) > E(W^*)$

\subsection{Sub-modularity}

\begin{equation}
    v(T \cup {t}) - v(T) \geq v(T \cup \{\bar{t},t\}) - v(T \cup \{\bar{t}\})
\end{equation}

\begin{align*}
    &v(T \cup {t}) - v(T) = \\ &\prod_{j=0}^{\alpha -1}\bar{\psi}_j \delta_t + (\bar{\psi}_t - 1)(\prod_{j = 0}^{\alpha - 1}\bar{\psi}_j \delta_\alpha + ... + \prod_{j = 0}^{p - 1}\bar{\psi}_j \delta_p)
\end{align*}
    


Let $\alpha < \beta$.

\begin{align*}
    & v(T \cup {\bar{t}, t}) - v(T \cup \{ \bar{t} \} ) = \\ & \prod_{j=0}^{\alpha -1}\bar{\psi}_j \delta_t + (\bar{\psi}_t - 1)(\prod_{j = 0}^{\alpha - 1}\bar{\psi}_j \delta_\alpha + ... + \prod_{j = 0}^{\beta - 1}\bar{\psi}_j \delta_{\bar{t}}) \\ & + \bar{\psi}_{\bar{t}}(\bar{\psi}_t - 1)(\prod_{j = 0}^{\beta - 1}\bar{\psi}_j \delta_\beta + ... + \prod_{j = 0}^{p - 1}\bar{\psi}_j \delta_{\bar{t}})
\end{align*}

Let $\beta < \alpha$

\begin{align*}
    & v(T \cup {\bar{t}, t}) - v(T \cup \{ \bar{t} \} ) = \\ &\bar{\psi}_{\bar{t}}(\prod_{j=0}^{\beta - 1}\bar{\psi}_j \delta_t + ... + \prod_{j=0}^{\alpha - 1}\bar{\psi}_j \delta_{\bar{t}}) \\ &+ \bar{\psi}_{\bar{t}}(\bar{\psi}_t - 1)(\prod_{j = 0}^{\alpha - 1}\bar{\psi}_j \delta_\alpha + ... + \prod_{j = 0}^{p - 1}\bar{\psi}_j \delta_{\bar{t}})
\end{align*}

\begin{problem}
 Single-Agent Risk-Aware Task Allocation Across Heterogeneous Days
\end{problem}

\begin{equation}
    E_j = \sum_{i=1}^p\sum_{m=0}^{\mu_\text{max}}r_{i,m}\psi_{i,m}-\theta(1-\psi_p) + E_{j+1}  \psi_p
\end{equation}



\begin{corollary}
Ordering of Cycles by reward to risk ratio on any given day is still optimal. \label{cor:ordering_of_cycles}
\end{corollary}

\begin{proposition}
Consider a set of tasks, $T = \{ t_1, t_2, ..., t_n \}$, assigned to an agent. If the agent is restricted to one-shot cycles, then taking any task whose reward to risk ratio is greater than $\theta + E_{j+1}$ will improve the expected reward. \label{prop:keep_good_r2r}
\end{proposition}

\begin{proof}
We will prove this by contradiction. Assume it is optimal to not take a task where $\frac{r_k \bar{\psi}_k}{1 - \bar{\psi}_k} > \theta + E_{j+1}$. Then, $E_j$ is optimal without it:

\begin{equation}
    E_j = \sum_{i=1}^pr_{i}\psi_{i}-\theta(1-\psi_p) + E_{j+1}  \psi_p
\end{equation}
Construct a new walk, $W*$, that includes a task $t_k$ as the last cycle and $\frac{r_k \bar{\psi}_k}{1 - \bar{\psi}_k} > \theta + E_{j+1}$. Note that by Corollary \ref{cor:ordering_of_cycles}, we know the optimal placement of this cycle. So, the overall expected reward can only improve by placing this cycle in the correct spot. Regardless, we denote the new expected reward as:
\begin{equation}
    E^*_j = \sum_{i=1}^pr_{i}\psi_{i} + r_k\bar{\psi}_k\psi_p -\theta(1-\psi_p\bar{\psi}_k) + E_{j+1}\psi_p\bar{\psi}_k
\end{equation}

By assuming $E_j$ is optimal, then $E^*_j - E_j < 0$.

\begin{equation}
    E^*_j - E_j = \psi_p(r_k\bar{\psi}_k - (E_{j+1} + \theta )(1 - \bar{\psi}_k) )  
\end{equation}

But, $\frac{r_k \bar{\psi}_k}{1 - \bar{\psi}_k} > \theta + E_{j+1}$ implies that $E^*_j - E_j > 0$, so $E_j$ is suboptimal.

\end{proof}

\begin{proposition}
Consider an ordered set of tasks, $T = \{ t_1, t_2, ..., t_n \}$, assigned to an agent. The agent visits all tasks in order of reward to risk ratio and the expected reward is denoted $E^*_j$. Suppose we add a new task, $t_k$, to $T$ such that $\frac{r_k \bar{\psi}_k}{1 - \bar{\psi}_k} < \theta + E_{j+1}$ and the new expected reward is $E_j$. Then, $E^*_j > E_j$. I.e. adding a task whose reward to risk ratio is less than $\theta + E_{j+1}$ is always suboptimal.
\end{proposition}

\begin{proof}
We will prove this by contradiction and assume that $E_j$ is optimal. Then, $E_j - E^*_j > 0$. By applying Proposition \ref{prop:keep_good_r2r} and Corollary \ref{cor:ordering_of_cycles}, then $t_k$ must go after all the tasks that satisfy $\frac{r_k \bar{\psi}_k}{1 - \bar{\psi}_k} > \theta + E_{j+1}$. 

\begin{equation}
    E_j - E^*_j = \psi_p(r_k\bar{\psi}_k - (E_{j+1} + \theta )(1 - \bar{\psi}_k) ) + (\psi_k - 1)(\sum_{i=l+1}^p r_{i}\psi_{i})
\end{equation}

However, we know by $\frac{r_k \bar{\psi}_k}{1 - \bar{\psi}_k} < \theta + E_{j+1}$ that the first term must be negative. The second term is always negative because $\psi_k \in [0,1]$. Therefore, $E_j - E^*_j < 0$ which contradicts the optimality of $E_j$.

\end{proof}

==> isomorphism_proof.tex <==
\subsubsection{Isomorphism to Probability of Failure Per Unit Distance}
We show an isomorphism between a previous drone routing formulation to our general case. 
\begin{align*}
    \max_{C\in \mathcal{C}}E(C(W)) = \max_{C\in \mathcal{C}} \sum_{i = 0}^{p} \sum_{m = 0}^{\mu_i} r_{i,m} \psi_{i,m} - \theta(1 - \psi_p)
\end{align*}

\begin{align*}
    \max_{W\in \mathcal{W}}E(W) = \max_{W\in \mathcal{W}} \sum_{i = 0}^{p} \sum_{m = 0}^{\mu_i} & r_{i,m} \phi^{\log_\phi \psi_{i,m}} \\ & - \theta(1 - \phi^{\log_\phi{\psi_p}})
\end{align*}

\begin{align*}
    \log_\phi{\psi_{i,m}} & = \log_\phi { \prod_{j \leq i, m < \mu_j} \rho(W_{j,m}, W_{j, m+1}) } \\ & = \sum_{j \leq i, m < \mu_j} \log_\phi{\rho(W_{j,m}, W_{j, m+1})}
\end{align*}

By defining $d_{i,j} = -\log_\phi \rho(i,j)$ and $d_k = -\log_\phi{\bar{\phi}_k}$, then $d_{i,j}$ can be interpreted as the distance between tasks $i$ and $j$ and $d_k$ is the total distance of cycle $k$. Then, $\phi$ is the probability of failure per unit distance.

\begin{align*}
    \max_{W\in \mathcal{W}}E(W) = \max_{W\in \mathcal{W}} \sum_{i = 0}^{p} \sum_{m = 0}^{\mu_i} & r_{i,m} \phi^{\sum_{k=1}^{i-1}d_k}\phi^{\sum_{j=1}^m d_{i,j}} \\ & - \theta(1 - \phi^{d_p})
\end{align*}

Inverting this substitution to show an isomorphism is straightforward from the other direction as well.

\begin{lemma}
Consider a weighted graph, $G = (V,E)$, where $V = T \cup \{t_0\}$ and $E = \{ (t_u, t_v) : t_u, t_v \in V, t_u \ne t_v \}$.  Each edge $e = (t_u,t_v) \in E$ has a weight $w(e) = w(t_u,t_v)$ denoting the distance between tasks $t_u$ and $t_v$. Let each triplet of edges in $E$ satisfy the triangle inequality, i.e. $w(t_u,t_v) + w(t_v,t_k) > w(t_u, t_k)$. Define $\phi \in (0,1)$ to be the probability of success per unit distance of every agent. Then, there exists an isomorphism between the problem of traversing $V$ to maximize the reward from , 
\end{lemma}

 Then, the probability the agent is able to travel from $t_u$ to $t_v$ is $\phi^{w(t_u,t_v)}$. More generally, the probability of traversing a walk is $\phi^{d}$ where $d$ is the total distance of the walk. Using this notation, we can map our version of SARATE to the metric space version.

\begin{align*}
    \max_{C\in \mathcal{C}}E(C(W)) = \max_{C\in \mathcal{C}} \sum_{i = 0}^{p} \sum_{m = 0}^{\mu_i} r_{i,m} \psi_{i,m} - \theta(1 - \psi_p)
\end{align*}

\begin{align*}
    \max_{W\in \mathcal{W}}E(W) = \max_{W\in \mathcal{W}} \sum_{i = 0}^{p} \sum_{m = 0}^{\mu_i} & r_{i,m} \phi^{\log_\phi \psi_{i,m}} \\ & - \theta(1 - \phi^{\log_\phi{\psi_p}})
\end{align*}

\begin{align*}
    \log_\phi{\psi_{i,m}} & = \log_\phi { \prod_{j \leq i, m < \mu_j} \rho(W_{j,m}, W_{j, m+1}) } \\ & = \sum_{j \leq i, m < \mu_j} \log_\phi{\rho(W_{j,m}, W_{j, m+1})}
\end{align*}

By defining $d_{i,j} = -\log_\phi \rho(i,j)$ and $d_k = -\log_\phi{\bar{\phi}_k}$, then $d_{i,j}$ can be interpreted as the distance between tasks $i$ and $j$, i.e., $w({i,j})$, and $d_k$ is the total distance of cycle $k$. Then, $\phi$ is the probability of failure per unit distance.

\begin{align*}
    \max_{W\in \mathcal{W}}E(W) = \max_{W\in \mathcal{W}} \sum_{i = 0}^{p} \sum_{m = 0}^{\mu_i} & r_{i,m} \phi^{\sum_{k=1}^{i-1}d_k}\phi^{\sum_{j=1}^m d_{i,j}} \\ & - \theta(1 - \phi^{d_p})
\end{align*}

Inverting this process to show an isomorphism is straightforward from the other direction as well. Construct a distance between tasks such that $\phi^{w(t_u,t_v)} = \rho(t_u,t_v)$. Because $\log \rho(t_u,t_v)$ satisfies the triangle inequality, the edges in $G$ also satisfies the triangle inequality for every triplet of tasks in $T$. 

Because the two problems are isomorphic, their optimal solutions are also isomorphic. Here we define an important relationship for choosing tasks on any given day.

==> multi_agent_case.tex <==

\section{Multi-Agent Case}

\subsection{Multi-Agent Formulation of the Bellman Equation}
Now, we move on to derive the Bellman equation for the multi-agent case, (i.e., $R > 1$.) We will come back to (\ref{eq:inductive_expected_reward_RSPD}) The goal of the team of agents is to solve the following problem:

\begin{problem}
 Risk-Aware Team Package Delivery (RTPD)
\end{problem}
 \begin{equation}
    \text{Find   } \text{arg}\max_{\mathcal{C}_1,\ldots,\mathcal{C}_K} \sum_{\mathcal{C}_h \in \mathcal{C}}\sum_{\beta \leq R} E(\mathcal{C}_h | \alpha_h = \beta)P(\alpha_h = \beta)
    \label{eq:RTPD}
\end{equation}

 Let $P(\alpha_{h+1} = \beta' | \alpha_{h} = \beta )$ be the conditional probability of having $\beta'$ agents survive epoch $h$ if $\beta$ agents were available at the depot at the start of the epoch. $P(\alpha_{h+1} = \beta' | \alpha_{h} = \beta )$ can be calculated by taking the probability of finishing the epoch for each agent as a trial in a Poisson Binomial distribution. 

\begin{definition}[Poisson Binomial Distribution]
 Consider a set of $\alpha$ independent random trials $X = \{\rho_1, \rho_2, \ldots, \rho_\alpha\}$, where the outcome of each trial $\rho_m \in X$ is a success or failure with probabilities $\rho_m$ and $(1 - \rho_m)$, respectively. Then, the probability that $\beta \leq \alpha$ of the trials are successful $P(\beta | \alpha)$ is calculated by the Poisson binomial distribution. 
%\begin{equation}
%    P(\beta | \alpha) = \frac{1}{\alpha - 1} \sum_{l = 0}^\alpha{e^{ -\beta l \frac{2i \pi}{\alpha + 1}}} \prod_{m = 1}^\alpha(1 + (e^{l \frac{2i \pi}{\alpha+ 1}}-1)\psi_{m} )
%    \label{eq:poisson}
%\end{equation}

\begin{equation}
    P(\beta | \alpha) = \sum_{Y \in X_\beta}\prod_{x_i \in Y}\rho_i \prod_{x_j \in Y^c}(1 - \rho_j)
    \label{eq:poisson}
\end{equation}
Where $X_\beta$ is all ways of choosing $\beta$ successful trials from $X$ and $Y^c$ is the complement of $Y$. Note that this combinatorial version of the Poisson binomial distribution is more intuitive, but the Fourier transform version is more computationally tractable[reference].
\end{definition}

\begin{corollary}
Consider a set of agents $\mathcal{A}$ available at the start of epoch $h$, each assigned a unique tour in $\mathcal{C}_{h,\alpha_h}$. Let $\bar{\rho}_{i,p}$ be the probability that agent $i \in \mathcal{A}$ can survive their tour $C_i \in  \mathcal{C}_{h,\alpha_h}$. The probability that $\beta' \leq \alpha_h$ agents survive for epoch $h + 1$ can be calculated by a Poisson binomial distribution, $P(\alpha_{h+1} = \beta' | \alpha_{h} = \beta )$ over the set of trials $\{ \bar{\rho}_{1,p}, \bar{\rho}_{2,p}, \ldots, \bar{\rho}_{\alpha_h,p}\}$. 
\end{corollary}

For the sake of simple notation, we shorten $P(\alpha_{h+1} = \beta' | \alpha_{h} = \beta )$ to $P_h(\beta'|\beta)$.

\begin{lemma}
Given an instance of $RTPD$, the conditional expected reward for a team of $\beta$ agents to accomplish their set of ordered walks during epoch $h$ is given by:

\begin{align}
    &E(\mathcal{C}_h | \alpha_h = \beta) = \label{eq:multiagent_conditional_expectation} \\ & \sum_{C_{\beta} \in \mathcal{C}_{h,\beta}}\sum_{W_i \in C_{\beta}}r_i\psi_i \nonumber - \theta \sum_{\beta' \leq \beta} P_h(\beta' |\beta )(\beta - \beta') \nonumber
\end{align}
\end{lemma}


One can easily verify that (\ref{eq:multiagent_conditional_expectation}) reduces to (\ref{eq:RSPD_1epoch_expectation}) if $\alpha_h = 1$. Furthermore, to calculate $P(\alpha_h = \beta_h)$ from (\ref{eq:RTPD}) more explicitly, we can use the law of total probability and substitute $P_h(\beta'|\beta)$ for $P(\alpha_{h+1} = \beta' | \alpha_{h} = \beta )$ to obtain the following definition.

\begin{definition}[Probability of $\beta$ Agents Surviving to a Given Epoch]
\begin{equation}
    P(\alpha_h = \beta_h) =  
 \sum_{ \beta_{h-1} \leq \ldots \beta_{2} \leq R} P_{h-1}(\beta_h | \beta_{h-1}) \ldots P_1(\beta_2 | R) \label{eq:prob_survival_to_epoch}
\end{equation}
\label{def:prob_survival_to_epoch}
\end{definition}

Substituting (\ref{eq:prob_survival_to_epoch}) into (\ref{eq:RTPD}) reveals a telescopic general form which can be optimized by dynamic programming. 

\begin{align}
    &\sum_{h \leq k} E_h(\mathcal{C}_h) = E(\mathcal{C}_{1,R} | \alpha_1 = R) + \label{eq:sub_general_form} \\ & \sum_{\beta_2 \leq R}P_{1}(\beta_2|R)\left(E(\mathcal{C}_{2,\beta_1}|\alpha_2 = \beta_2) + \sum_{\beta_3 \leq \beta_2}P_{2}(\beta_3|\beta_2)(\ldots)\right)  \nonumber
\end{align}



The expected reward for the epoch is telescopic with respect to the expected reward for the remaining epochs. In other words, the terms inside the telescoping parentheses at level $h - 1$ are exactly equal to the expected reward for an instance of RTPD of only the remaining $k - h$ epochs. This fact means we can define a Bellman equation which optimizes (\ref{eq:sub_general_form}). Let $V_h(\beta)$ be the maximum expected reward for an epoch of only epochs $h$ to $k$ if $\beta$ agents are available on epoch $h$. 

\begin{definition}[Bellman Equation for RTPD]
\begin{align}
    V_h(\beta) = \max_{\mathcal{C}_{h,\beta}} & E(\mathcal{C}_{h,\beta} | \alpha_h = \beta) \label{eq:Bellman_eq} \\ &+ \sum_{\beta' \leq \beta}P_h(\beta'|\beta) (V_{h+1}(\beta') - \theta(\beta - \beta')) \nonumber
\end{align}

\begin{equation}
    V_k(\beta) = \max_{\mathcal{C}_{k,\beta}} \bar{E}(\mathcal{C}_{k,\beta})
    \label{eq:Bellman_eq_base}
\end{equation}
\label{def:bellman_eq_RAMAHP}
\end{definition}

%There are two special cases of RTPD that are worth analysis. 

%We will restrict the remainder of this paper to analysis of a special case of RTPD where each agent can only deliver one package at a time, i.e. $\mu = 1$.



%For the sake of intuition, we will restrict ourselves to a package delivery scenario. simplicity, we will assume that the reward for all tasks in a closed walk are given before the beginning of the next closed walk, i.e. $\psi_{i,m} < \psi_{j,m'}$ for any $t_{i,m}$ and $t_{j,m'}$ if $i < j$.


%There are two alternative scenarios we consider for when a reward is given. Either the rewards are given upon accomplishing a task, i.e. a package delivery scenario, or they are given during the rest state, i.e. a package collection scenario. The expected reward for each scenario is similar. The properties we prove in this work do not rely on either scenario, however the package delivery scenario maintains the general form. In fact, the package collection scenario can be seen as a restriction on the package delivery scenario by assigning the probability of receiving a task to be the same as the probability of completing the cycle.

%\subsection{Package Delivery Scenario}
%Impose a maximum number of tasks an agent can accomplish before resting to obtain more packages by an upper limit on the cycles, $\mu_\text{max}$.
%\begin{equation}
%    E(C(W)) = \sum_{i=1}^p\sum_{m=0}^{\mu_\text{max}}r_{i,m}\psi_{i,m}-\theta(1-\psi_p)
%\end{equation}

%\subsection{Package Collection Scenario}
%By imposing $\forall m \leq \mu_i : \psi_{i,m} = \psi_{i}$, then $\sum_{m=0}^{\mu_i}r_{i,m}\psi_{i,m} = R_i\psi_i$ where $R_i = \sum_{m=0}^{\mu_i}r_{i,m}$.
%\begin{equation}
%    E(C(W)) = \sum_{i=1}^p R_{i}\psi_{i}-\theta(1-\psi_p)
%\end{equation}
%This scenario is equivalent to the problem presented in \cite{Prasad_A_2019_Risk_Aware}.

%\begin{problem}
% Single-Agent Risk-Aware Task Execution (SARATE)
%\end{problem}

%\begin{equation}
%    \text{Find   } W* \in \text{arg}\max_{W \in \mathcal{W}} E(C(W))
%\end{equation}

\subsection{Analysis}
Given $k$ agents available on the first day, we want to maximize the expected reward across all remaining days. Let $E_i(k)$ be the expected reward on day $i$ for walk $W_{i,k}$ if we have $k$ drones on day 1.

\begin{problem}
 Multi-Agent Task Allocation Across Heterogeneous Days (MARATAAHD)
\end{problem}

\begin{equation}
     E(h) = \max_{\{ W_{1,1...k}, W_{2,1...k}, ..., W_{h,1...k} \}} \sum_{i = 1}^{h} E_i(k, C(W_{i,1...k}))
\end{equation}

\begin{equation}
    V_n(k) = R_n(k) + \theta \sum_{j \leq k}P_n(j|k)((k-j))
\end{equation}

\begin{equation}
    V_g(k) = R_g(k) + \sum_{j \leq k}P_i(j|k)( V_{g+1}(j) - \theta(k-j))
\end{equation}

\begin{align*}
    P(j|k) &= P( \text{Remaining Agents} = j) \\ &= \frac{1}{k - 1} \sum_{l = 0}^k{e^{ -jl \frac{2i \pi}{k + 1}}} \prod_{m = 1}^k(1 + (e^{l \frac{2i \pi}{k + 1}}-1)\psi_{m,\mu_m} )
\end{align*}
    
\begin{align*}
    P(j|k) - P(j|k) = \frac{1}{k - 1} \sum_{l = 0}^k{e^{ -jl \frac{2i \pi}{k + 1}}} \prod_{m = 1}^k(1 + (e^{l \frac{2i \pi}{k + 1}}-1)\psi_{m,\mu_m} )
\end{align*}



\begin{equation}
    \frac{R_t\psi_t}{(1 - \psi_t)} > \Tilde{P}_g(j|k) (V_{g+1}(j) - \theta(k - j))
\end{equation}



Always maximize the overall reward for today and the remaining days.

\begin{definition}[Marginal Gain]
Consider a new package delivery $W_i$ to be added as the final cycle in $C_m$ assigned to agent $m$ during epoch $h$. Then, we define the marginal gain from adding package $W_i$ to $C_m$ to be:
\begin{equation}
    \delta_{m,i} = r_t \sqrt{\rho_t} - (1 - \rho_t)\sum_{\beta \leq \alpha}\Tilde{P}_{W_i}(\beta | \alpha)(V_{h+1} - \theta(\alpha - \beta))
\end{equation}
\end{definition}


\begin{lemma}
\begin{equation}
    V_h(\beta) = \sum_{C_{m} \in \mathcal{C}_{h,\beta}}\sum_{W_i \in C_{m}} \bar{\rho}_{i-1} \delta_{m,i}
\end{equation}
\end{lemma}
\begin{proof}

\begin{align}
    V_h(\beta) =& \sum_{C_{m} \in \mathcal{C}_{h,\beta}}\sum_{W_i \in C_{m}} r_i \psi_i \\& + \sum_{\beta' \leq \beta}
    P_h(\beta'|\beta) (V_{h+1}(\beta') - \theta(\beta - \beta')) \nonumber
\end{align}

\begin{equation}
    \sum_{C_{m} \in \mathcal{C}_{h,\beta}}\sum_{W_i \in C_{m}} r_i \psi_i = \sum_{C_{m} \in \mathcal{C}_{h,\beta}}\sum_{W_i \in C_{m}} \bar{\rho}_{i-1} r_i \sqrt{\rho_i}
\end{equation}
Let $P_{W_{q}}(\beta'|\beta)$ be the Poisson binomial distribution of $\mathcal{C}_{h,\beta}$ if we remove the set $\{W_q,W_{q+1},..., W_{p}\}$ from $C_{m} \in \mathcal{C}_{h,\beta}$.
\begin{align*}
    P_h(\beta'|\beta) &= P_h(\beta'|\beta) - P_{W_p}(\beta'|\beta) \\ &+ P_{W_p}(\beta'|\beta) - P_{W_{p-1}}(\beta'|\beta) \\ &+ P_{W_{p-1}}(\beta'|\beta) ... - P_{W_2}(\beta'|\beta) \\ &+ P_{W_2}(\beta'|\beta) )
\end{align*}
Then, we can use the alternative Poisson quotient difference identity, $P_h(\beta'|\beta) - P_{W_p}(\beta'|\beta) = \Tilde{P}_{W_p}(\beta'|\beta)(\rho_p - 1)\bar{\rho}_{p-1}$ to construct the following:

\begin{align*}
    V_h(\beta) =\\ \sum_{C_{m} \in \mathcal{C}_{h,\beta}}&\sum_{W_i \in C_{m}} \bar{\rho}_{i-1} r_t \sqrt{\rho_t} \\&- \bar{\rho}_{i-1}(1 - \rho_i)\sum_{\beta \leq \alpha}\Tilde{P}_{W_i}(\beta | \alpha)(V_{h+1} - \theta(\alpha - \beta)) ) \\  &= \sum_{C_{m} \in \mathcal{C}_{h,\beta}}\sum_{W_i \in C_{m}} \bar{\rho}_{i-1} \delta_{m,i}
\end{align*}

\end{proof}

\subsection{Submodularity of RTPD}
We say a set function, e.g. $v(T)$, is submodular if the following condition holds:

\begin{equation}
    v(T \cup {t_s}) - v(T) \geq v(T \cup \{t_r,t_s\}) - v(T \cup \{t_r\})
    \label{eq:submodularity}
\end{equation}

Submodularity is a very useful property which can prove approximation ratios on greedy algorithms. Here we will prove that the expected reward for any instance of RTPD is submodular. 

\begin{lemma}
$V_h(\beta)$ is submodular for all packages which satisfy (\ref{eq:reward_to_risk_ratio_bound}).
\end{lemma}

\begin{proof}
$V_h(\beta)$ is broken up into two parts and if both parts are submodular then the overall expression is submodular.

\begin{enumerate}
    \item $\sum_{\beta' \leq \beta} P_h(\beta'|\beta) (V_{h+1}(\beta') - \theta(\beta - \beta')) $ \label{submod:part_1} 
    \item $E(\mathcal{C}_{h,\alpha_h}| \alpha_h)$ \label{submod:part_2}
\end{enumerate}

We will prove part \ref{submod:part_1} is submodular, then part \ref{submod:part_2}. Intuitively, by increasing the tour length of agent $m$, the probability that the agent survives decreases. The definition of the Poisson binomial distribution follows this intuition and it is monotonic with respect to each agents probability of survival, which decreases with tour length. Therefore, part \ref{submod:part_1} must be submodular because as more packages are added to $\mathcal{C}_{h,\beta}$ the tour length increases.

Consider two package deliveries $\{ W_r\}$ and $\{ W_s\}$ to be added to tour $C_m \in \mathcal{C}_{h,\alpha_h}$ assigned to agent $m$. Assume the reward-to-risk ratios $\gamma_r$ and $\gamma_s$ satisfy Lemma \ref{lem:reward_to_risk_ratio_bound} when included in $C_m$ so that the marginal gains $\delta_r$ and $\delta_s$ will be positive. Let $\mathcal{C}_{h,\alpha_h} \cup \{W_r\}$ be shorthand for appending delivery $W_t$ to tour $C_m$ for agent $m$. Finally, let the indeces $k$ and $l$ be the indeces for where $\{ W_r\}$ and $\{ W_s\}$ are inserted into $C_m$, respectively.
\end{proof}

\begin{align}
     E(\mathcal{C}_{h,\alpha_h} \cup& \{W_r\} | \alpha_h) = \label{eq:submod_E_add_W_r}\\ & \delta_1 + \ldots \bar{\rho}_{k-1} \delta_r + (\rho_r )[\bar{\rho}_{k-1} \delta_{k} + ... + \bar{\rho}_{p-1}\delta_p] \nonumber
\end{align}

\begin{align}
    MG_{r} = E(\mathcal{C}_{h,\alpha_h} \cup& \{W_r\} | \alpha_h) - E(\mathcal{C}_{h,\alpha_h} | \alpha_h) = \label{eq:submod_add_W_r}\\ & \bar{\rho}_{k-1} \delta_r + (\rho_r - 1)[\bar{\rho}_{k-1} \delta_{k} + ... + \bar{\rho}_{p-1}\delta_p] \nonumber
\end{align}
    

Let $k < l$.

\begin{align}
    & MG_{r,s} = E(\mathcal{C}_{h,\alpha_h} \cup \{W_r, W_s\} | \alpha_h) - E(\mathcal{C}_{h,\alpha_h} \cup \{ W_{s} \} | \alpha_h) \label{eq:submod_add_both}\\ & = \bar{\rho}_{k-1} \delta_r + (\rho_r - 1)(\bar{\rho}_{k-1}\delta_k + ... + \bar{\rho}_{l-2} \delta_{l - 1} + \bar{\rho}_{l-1} \delta_{s})  \nonumber \\ & + \rho_s(\rho_{r} - 1)(\bar{\rho}_{l-1} \delta_l + ... + \bar{\rho}_{p-1} \delta_{p}) \nonumber
\end{align}

Taking the difference between (\ref{eq:submod_add_W_r}) and (\ref{eq:submod_add_both}) we obtain:

\begin{align}
    MG_{r,s} - MG_r &= (\rho_r - 1)(\bar{\rho}_{l-1}\delta_s)  \nonumber \\ &  
     + (\rho_s - 1)(\rho_r - 1)(\bar{\rho}_{l-1}\delta_l + ... + \bar{\rho}_{p-1}\delta_p) \nonumber
\end{align}

\begin{equation}
    = (\rho_r - 1)\bar{\rho}_{l-1}[\delta_s + (\rho_s - 1)(\delta_l + \ldots \prod_{j = l}^{p - 1}\rho_{j}\delta_p)]
     \label{eq:submod_diff_Wrs_Wr}
\end{equation}

The terms in the square brackets equal the marginal gain from adding $W_s$ to the set of cycles $\{ W_k, W_{k+1}, ... ,W_p\}$. Assuming $\delta_s$ is positive, then these terms, along with $\bar{\rho}_{l-1}$, will be positive. However, $(\rho_r - 1) < 0$. So, overall  $MG_{r,s} - MG_r < 0$ which satisfies (\ref{eq:submodularity}). Now, we consider the opposite case where $l < k$.

\begin{align*}
    MG_{s,r}&=E(\mathcal{C}_{h,\alpha_h} \cup \{W_{r}, W_s\} | \alpha_h) - E(\mathcal{C}_{h,\alpha_h} \cup \{ W_{s} \} | \alpha_h) \\ & = \rho_s \delta_r + \rho_s(\rho_r - 1)(\bar{\rho}_{k-1} \delta_k + ... + \bar{\rho}_p \delta_{p}) \\ &= \rho_s(MG_{r}) < MG_{r}
\end{align*}

Therefore, both cases satisfy (\ref{eq:submodularity}) which means $E(\mathcal{C}_{h,\alpha_h} | \alpha_h)$ is submodular.


\subsection{Bounds on Reward-to-Risk Ratio of Optimal Cycles}
Naturally, we want to derive a way of determining which cycles are worth following and which are not. 

\begin{definition}[Poisson Quotient Different]
Consider the Poisson binomial distribution $P_h(\beta'|\alpha_h)$ calculated by the set of tours $\mathcal{C}_{h,\alpha_h}$ for a given epoch $h$. Let $C_m \in \mathcal{C}_{h,\alpha_h}$ be a tour for agent $m \in \mathcal{A}_h$. $W_i$ is a new package delivery to be added to $C_m$ and we denote the new tour as $C'_m = C_m \cup W_i$. We say $P'_{h}(\beta'|\alpha_h)$ is the new Poisson binomial distribution for epoch $h$ when using $C'_m$ instead of $C_m$. Then, $\rho'_m$ is the probability that agent $m$ finishes $C'_m$ while $\rho_m$ is the same for $C_m$. Finally, we define the Poisson quotient difference between the two distributions to be:

\begin{equation}
    \Tilde{P}_{W_i}(\beta|\alpha_h) = \frac{P'_{h}(\beta | \alpha) - P_{h}(\beta | \alpha)}{(\bar{\rho}'_m - \bar{\rho}_m)}
\end{equation}
We can also extend an equivalent definition of $\Tilde{P}_{W_i}(\beta|\alpha_h)$ where we begin with an initial tour $C_m$ and we consider the quotient difference between $C_m$ and the set of all cycles before $W_i \in C_m$.
\end{definition}



\begin{corollary}
Let $\Gamma = \{ \bar{\rho}_1, \bar{\rho}_2, \ldots, \bar{\rho}_{\alpha_h} \} \backslash \bar{\rho}_m$ be the set of probabilities for each agent $j \in \mathcal{A}_h \backslash m$ to finish tour $C_j \in \mathcal{C}_{h,\alpha_h}$. By using the discrete Fourier transform of (\ref{eq:poisson}), one can easily show that the Poisson quotient difference is a function of all probabilities in $\Gamma$ without $\bar{\rho}_m$. \label{cor:constant_P_tilde}
\end{corollary}


\begin{lemma}
Assume that $\alpha_h$ agents have survived to epoch $h$. Let $C'_m \in \mathcal{C}'_{h,\alpha_h}$ be the optimal tour for agent $m$ during epoch $h$. Choose any cycle, $W_i \in C'_m$ and construct a new tour $C_m$ by taking out all cycles after and including $W_i$. Let $\Tilde{P}_{W_i}$ be the Poisson quotient difference between tour $C'_m$ and $C_m$. Then, the reward-to-risk ratio $\gamma_i$ of cycle $W_i$ must satisfy the following inequality to be optimal:

\begin{equation}
    \gamma_i > \sum_{\beta' \leq \alpha_h} \Tilde{P}_{W_i}(\beta'|\alpha_h) (V_{h+1}(\beta') - \theta(\alpha_h - \beta'))
    \label{eq:reward_to_risk_ratio_bound}
\end{equation}
\label{lem:reward_to_risk_ratio_bound}
\end{lemma}

\begin{proof}
We will prove this by contradiction. Suppose there exists a cycle, $\bar{W} \in C_m$, whose reward-to-risk ratio is: 
\begin{equation}
    \bar{\gamma} < \sum_{\beta \leq \alpha}\Tilde{P}_{\bar{W}}(\beta'|\alpha_h)(V_{h+1}(\beta') - \theta(\alpha_h - \beta')) \label{eq:lem_lesser_bound_r2r}
\end{equation} By Corollary \ref{cor:constant_P_tilde}, $\Tilde{P}_{W_i}(\beta|\alpha)$ is constant for any change to $C_m$. Additionally, by applying \ref{eq:lem_lesser_bound_r2r} and assuming all other cycles in $C_m$ satisfy (\ref{eq:reward_to_risk_ratio_bound}), $\bar{\gamma}$ must be less than $\gamma_i$ for all $W_i \in C_m \backslash \bar{W}$. Furthermore, Lemma $\ref{lem:ordering_of_cycles}$ implies that $\bar{W}$ must be the last cycle in $C_m$. However, by calculating  $E(\mathcal{C}'_{h,\alpha_h} | \alpha_h) - E(\mathcal{C}_{h,\alpha_h} | \alpha_h)$ we can see that $E(\mathcal{C}_{h,\alpha_h} | \alpha_h) > E(\mathcal{C}'_{h,\alpha_h} | \alpha_h)$ which contradicts the optimality of $C'_m$. Let $r'$ and $\psi'$ be the reward and probability of obtaining $r'$, respectively, for $\bar{W}$.

\begin{align*}
    E(\mathcal{C}'_{h,\alpha_h} | \alpha_h) &- E(\mathcal{C}_{h,\alpha_h} | \alpha_h) = r' \psi' \\ + & \sum_{\beta \leq \alpha} (\bar{\rho}'_m - \bar{\rho}_m)\Tilde{P}_{\bar{W}}(\beta|\alpha)(V_{h+1}(\beta) - \theta(\alpha - \beta))
\end{align*}

By noting that $\bar{\rho}'_m = \rho'\bar{\rho}_m$ and $(\bar{\rho}'_m - \bar{\rho}_m) = \bar{\rho}_m(1 - \rho'_m)$, we can obtain:
\begin{align*}
    E(\mathcal{C}'_{h,\alpha_h} | \alpha_h) &- E(\mathcal{C}_{h,\alpha_h} | \alpha_h) = \bar{\rho}_m r' \psi' \\ - & \bar{\rho}_m\sum_{\beta \leq \alpha} (1 - \bar{\rho}'_m)\Tilde{P}_{\bar{W}}(\beta|\alpha)(V_{h+1}(\beta) - \theta(\alpha - \beta))
\end{align*}
 which is positive only if $\bar{\gamma}$ contradicts  (\ref{eq:lem_lesser_bound_r2r}).
\end{proof}




\begin{algorithm}[h!]
\SetAlgoLined
\KwIn{An instance of RTPD}
\KwResult{A collection of tours $\mathcal{C}$ that solves RTPD. }
Initialize $\mathcal{C} = \emptyset$\;
Let $T = \{t_1, t_2, \ldots, t_n\}$ be all possible packages in any order. For each package $t_i$ calculate $\gamma_i$ for $W_i$

 \For{each epoch $h < K$ and $\beta \leq R$}{
  Let $C_m \in \mathcal{C}_{h,\beta}$\;
  Find the agent $m$ and task $t_i \in T_h$ that maximal marginal gain $\sigma_{m,i}$\;
  $C_m \leftarrow C_m \cup W_i$\;
 }
 \caption{Greedy Solution to RTPD}
 \label{alg:RTPD}
\end{algorithm}

\begin{lemma}
The expected reward returned by algorithm \ref{alg:RTPD} for RTPD is lower-bounded by $2^{-K}$ of the optimal allocation.
\end{lemma}
\begin{proof}
Because $V_h(\beta)$ is a submodular welfare problem, a greedy solution will at worst achieve a $1/2$ approximation from optimal. So, each $V_h(\beta)$ must be at least $1/2 \bar{V}_h$
\end{proof}


==> multi_agent_same_tasks.tex <==
\section{Multi-Agent RSPD}
In this section, we will expand our definitions from RSPD to account for multiple agents and then show some of the difficulties with multi-agent RSPD. A team of $M$ homogeneous agents (e.g., drones) is available at the depot at the first epoch to deliver the packages to their desired locations. Since some agents may fail during each epoch, we denote the set of agents available at the start of epoch $h$ by $\mathcal{A}_h$, with $|\mathcal{A}_1| = M$ and $\mathcal{A}_{h+1} \subseteq \mathcal{A}_h$ for $h \in \{1, 2, \ldots, K-1\}$. Then, $\alpha_h = |\mathcal{A}_h|$. Furthermore, since agents are homogeneous, we denote $\mathcal{A}_{h} = \{1, 2, \ldots, \alpha_h\}$ without loss of generality (i.e., we can simply renumber all agents at the start of each epoch to have labels from $1$ to $\alpha_h$). Due to time constraints on the agents, the dispatcher preassigns package delivery plans for each agent at the start of the epoch. Let $C_{h,i}$ denote the set of package deliveries allocated to agent $i$ at epoch $h$. Agent $i$ then executes its assigned deliveries in each epoch in some order. If agent $i$ fails during their deliveries, the other agents do not pickup the leftover packages that agent $i$ could not get to and a cost of $\theta$ is incurred. Let $\mathcal{C}_{h_{\alpha_h}} = \{C_{h,1}, C_{h,2}, \ldots, C_{h,\alpha_h}\}$ be a set of disjoint tours allocated to the $\alpha_h$ agents that have survived to epoch $h$. We denote the probability of agent $m$ finishing the last package delivery cycle in epoch $h$ as $\bar{\rho}_{{h,m}}$. It is required that we allow for different $\bar{\rho}_{{h,m}}$ depending on the number of agents that survive to epoch $h$, however this will be baked into the definition to avoid cumbersome notation.
\begin{problem}
Multi-Agent RSPD
 \begin{equation}
    \text{Find   } \text{arg}\max_{\mathcal{C}_1,\ldots,\mathcal{C}_K} \sum_{h = 1}^{K}
    \sum_{m = 1}^{M}E(\mathcal{C}_{h} | \alpha_h = m )P(\alpha_h = m).
    \label{eq:HHRSPD}
\end{equation}
\end{problem}

\begin{equation}
    E(\mathcal{C}_{h} | \alpha_h = m ) = \sum_{i = 0}^p r_i \psi_i - \sum_{j = 0}^m P(\alpha_{h+1} = \beta-j|\alpha_h=\beta)(j \theta)
\end{equation}

\begin{definition}[Poisson Binomial Distribution]
 Consider a set of $\alpha$ independent random trials $X = \{\rho_1, \rho_2, \ldots, \rho_\alpha\}$, where the outcome of each trial $\rho_m \in X$ is a success or failure with probabilities $\rho_m$ and $(1 - \rho_m)$, respectively. Then, the probability that $\beta \leq \alpha$ of the trials are successful $P(\beta | \alpha)$ is calculated by the Poisson binomial distribution. 
%\begin{equation}
%    P(\beta | \alpha) = \frac{1}{\alpha - 1} \sum_{l = 0}^\alpha{e^{ -\beta l \frac{2i \pi}{\alpha + 1}}} \prod_{m = 1}^\alpha(1 + (e^{l \frac{2i \pi}{\alpha+ 1}}-1)\psi_{m} )
%    \label{eq:poisson}
%\end{equation}

\begin{equation}
    P(\beta | \alpha) = \sum_{Y \in X_\beta}\prod_{x_i \in Y}\rho_i \prod_{x_j \in Y^c}(1 - \rho_j)
    \label{eq:poisson}
\end{equation}
Where $X_\beta$ is all ways of choosing $\beta$ successful trials from $X$ and $Y^c$ is the complement of $Y$. Note that this combinatorial version of the Poisson binomial distribution is more intuitive, but the Fourier transform version is more computationally tractable[reference].
\end{definition}

\begin{corollary}
Consider a set of agents $\mathcal{A}$ available at the start of epoch $h$, each assigned a unique tour in $\mathcal{C}_{h,\alpha_h}$. Let $\bar{\rho}_{h,m}$ be the probability that agent $m \in \mathcal{A}$ can survive their tour $C_m \in  \mathcal{C}_{h,\alpha_h}$. The probability that $\beta' \leq \alpha_h$ agents survive for epoch $h + 1$ can be calculated by a Poisson binomial distribution, $P(\alpha_{h+1} = \beta' | \alpha_{h} = \beta )$ over the set of trials $\{ \bar{\rho}_{h,1}, \bar{\rho}_{h,2}, \ldots, \bar{\rho}_{h,\alpha_h}\}$. 
\end{corollary}

\begin{definition}
The probability that $\beta$ agents are available to deliver $t_i \in \mathcal{C}_h$.
\begin{equation}
    P(\alpha_{h,i} = \beta) = \sum_{m = \beta}^{M}P(\alpha_{h} = m)P(\alpha_{h,i} = \beta | \alpha_h = m)
\end{equation}

\begin{align}
    &P(\alpha_{h,i} = \beta | \alpha_h = m) = \\ &\sum_{j = 0}^{m - \beta}P(\alpha_{h,{i}} = \beta | \alpha_{h,{i-1}} = m - j)P(\alpha_{h,{i-1}} = m - j | \alpha_h = m) \nonumber \\
    &= \sum_{j = 0}^{m - \beta} (\rho_{h,i-1}^2)(1 - \rho_{h,i-1}^2)^{j} P(\alpha_{h,{i-1}} = m - j | \alpha_h = m)
\end{align}
\end{definition}

\begin{align}
    &P(\alpha_{h+1} = \beta |\alpha_h=m) = \\ &\sum_{j = 0}^{m - \beta} (\rho_{p_h}^2)(1 - \rho_{p_h}^2)^{m - j - \beta} P(\alpha_{h,{p}} = m - j | \alpha_h = m)
\end{align}

\begin{definition}
The probability $\psi_i$ of receiving reward $r_i$ for a package delivery $t_i \in \mathcal{C}_h$ is calculated by:

\begin{equation}
    \psi_i = \rho_i 
\end{equation}

\end{definition}

==> old_MDP_proofs.tex <==
To begin, first consider the state-space $S = \{x_1,x_2,x_3\}$ containing only three states where $x_1$ corresponds to the agent being alive, $x_2$ corresponds to the dispatcher incurring a cost $\theta$, and $x_3$ corresponds to the agent's failure. Define the action space $A$ as the set of all $n$-bit strings $A = \{0,1\}^n$ where $n$ is the number of tasks in an instance of IHRSPD. While the MDP is in the state $x_1$, the controller may treat each component $a_i$ of  $\mathbf{a} \in A$ as a bit that determines if package delivery $W_i$ is taken for the current epoch. For states $x_2$ and $x_3$, the rewards will be $-\theta$ and $0$, respectively, and remain constant with respect to $\mathbf{a}$. Now, we will define the reward and probability functions which achieve an isomorphism to IHRSPD under this class of policies. Consider the following continuous function for the probability of receiving a reward $r_i$ from a package delivery $W_i$ where the probability of success is $\rho_i$. 
\begin{equation}
    \bar{\phi}_i(a_i) = (1 - (1 - \rho_i)a_i)
\end{equation}

This function $\bar{\phi}_i : [0,1] \mapsto [\rho_i,1]$ is monotonic decreasing where $\phi_i(0) = 1$ and $\phi_i(1) = \rho_i$. Using this, we can construct the more general probability functions for the MDP.


\begin{definition}[MIHRSPD Probability Functions]
\begin{equation}
    \phi(i,\mathbf{a}) = \bar{\phi}_i(a_i)\prod_{j < i}\bar{\phi}_j(a_j)^2
\end{equation}
\begin{equation}
    \phi(\mathbf{a}) = \prod_{j = 1}^n\bar{\phi}_j(a_j)^2 \label{eq:MDP_prob_2}
\end{equation}
\end{definition}



%\begin{lemma}
%The MIHRSPD probability functions, $\bar{\phi}(i,a)$ and $\bar{\phi}(a)$ are continuous over $A$. 
%\end{lemma}
%\begin{proof}
%We say the function $\bar{\phi}: A \rightarrow \mathbb{R}$ is continuous for all points $x \in A$ if given any $\epsilon > 0$, there exists a $\delta > 0$ such that:
%\begin{equation}
%    \forall a \in A : |x - a| < \delta \implies | \bar{\phi}(x) - \bar{\phi}(a)  | < \epsilon
%\end{equation}
%In the case of the Hamming cube, the distance $|x - a|$ is specified by the Hamming distance, i.e., the number of unlike bits between two strings in $A$. 
%\end{proof}

From here, we can define the transition probabilities given any action vector $\mathbf{a}$. 
\begin{definition}[MIHRSPD Transition Probability Functions]
For all $\mathbf{a} \in A$,
\begin{equation}
    p_{1,1}(\mathbf{a}) = \phi(\mathbf{a}) = 1 - p_{1,2}(\mathbf{a})
\end{equation}
\begin{equation}
    p_{2,3}(\mathbf{a}) = p_{3,3}(\mathbf{a}) = 1
\end{equation}
For all other probability transition laws, $x,y \in S$:
\begin{equation}
    p_{x,y}(\mathbf{a}) = 0, \forall \mathbf{a} \in A.
\end{equation}
\label{def:MIHRSPD_P_Transition_Functions}
\end{definition}

Given these probability functions, the reward functions can be properly defined, followed by the MDP isomorphic to IHRSPD.

\begin{definition}[MIHRSPD Reward Functions]
For all $\mathbf{a} \in A$,
\begin{equation}
    R(x_1,\mathbf{a}) = \sum_{i=0}^n \alpha_i r_i \phi(i,\mathbf{a})
\end{equation}
\begin{equation}
    R(x_2,\mathbf{a}) = -\theta
\end{equation}
\begin{equation}
    R(x_3,\mathbf{a}) = 0
\end{equation}

\label{def:MIHRSPD_Reward_Functions}
\end{definition}

\begin{definition}[Markov-IHRSPD (MIHRSPD)]
An instance of MIHRSPD is given by the set $\mathcal{M} = \{\mathcal{I},H\}$ where $\mathcal{I}$ is an instance of IHRSPD and $H = (S,A,\{A(x)\},R,P)$ is a MDP defined as follows. Define the state-space $S = \{x_1,x_2,x_3\}$ with three states. Let the action space $A$ be the set of all n-bit strings $A = \{0,1\}^n$, where $n$ is the number of tasks $|\mathcal{T}|$ in $\mathcal{I}$. Define the compact action spaces $\forall x \in S : A(x) = A$. Let the reward and probability transition laws functions be specified by $\mathcal{I}$ using Definition \ref{def:MIHRSPD_Reward_Functions} and Definition \ref{def:MIHRSPD_P_Transition_Functions}. Then, the problem is to find a policy $\pi$ in the set of all policies $\mathcal{P}$ that solves

\begin{equation}
    \text{Find   } \text{arg}\max_{\pi \in \mathcal{P}}E^\pi_x\left[\sum_{h=1}^\infty R(X_h,A_h) \right].
    \label{eq:MIHRSPD_expected_reward}
\end{equation}

\end{definition}

\begin{definition}[Induced Package Delivery Plan]
Given an instance of $\mathcal{M} = \{\mathcal{I},H\}$ of MIHRSPD, consider any policy $\pi$ for MIHRSPD. We define an induced package delivery plan $\mathcal{C}$ as follows. For every epoch $h$, the package delivery plan $\mathcal{C}_h$ for epoch $h$ is constructed from the action vector $A_h = \pi(X_h = x_1)$ via the following:
\begin{equation}
    \mathcal{C}_h = \{ W_j | \forall t_j \in T : a_j \in A_h = 1 \}.
\end{equation}
\label{def:induced_package_delivery_plan}
\end{definition}

One can easily verify that the set of all possible induced package delivery plans is isomorphic to the set of all package delivery plans and action vectors. Furthermore, the probability $\phi(\mathbf{a})$ in (\ref{eq:MDP_prob_2}) given a state vector $\mathbf{a}$ is equal to the probability $\bar{\rho}_{q_h}$ of the the agent surviving the induced package delivery plan $\mathcal{C}_h$ for epoch $h$ constructed from $\mathbf{a}$. 

From here, we can show that the expected reward for MIHRSPD is equal to the expected reward for an instance of IHRSPD

\begin{lemma}
Consider an instance $\mathcal{M} = \{\mathcal{I},H\}$ of MIHRSPD constructed from an instance of IHRSPD $\mathcal{I}$. Given any policy $\pi$ that solves $\mathcal{M}$, construct its induced package delivery plan $\mathcal{C}$. Then, the expected reward for $\mathcal{M}$ beginning in state $x_1$ with policy $\pi$ equals the expected reward for IHRSPD with plan $\mathcal{C}$.
\label{lem:MIHRSPD_equals_IHRSPD}
\end{lemma}

\begin{proof}
We will begin by expanding the expected reward for MIHRSPD explictly. Note for notational brevity, we have omitted the proper notation $R(X_h = x_i, A_h = \pi(x_i))$ for $R(x_i,\pi(x_i))$ but the $h$ dependence is always implied. We have,
\begin{align}
    E^\pi_x&\left[\sum_{h=1}^\infty R(X_h,A_h) \right] \nonumber = \sum_{h=1}^\infty \sum_{i=1}^3 R(x_i,\pi(x_i))P(X_h = x_i) \\ &= \sum_{i=1}^3 \sum_{h=1}^\infty R(x_i,\pi(x_i))P(X_h = x_i) .
\end{align}

Breaking the inner summation into three parts, one for each state, we can construct an infinite sum for each state. First, consider the ``dead'' state, $x_3$. Because $\forall \mathbf{a} \in A(x_3) : R(x_3,\mathbf{a}) = 0$, its infinite sum is completely removable, i.e.,
\begin{equation}
    \forall \pi \in \mathcal{P} : \sum_{h=1}^\infty R(x_3,\pi(x_3))P(X_h = x_3) = 0.
\end{equation}

Therefore, we are left with 

\begin{align}
    E^\pi_x\left[\sum_{h=1}^\infty R(X_h,A_h) \right] & = 
    \sum_{h=1}^\infty R(x_1,\pi(x_1))P(X_h = x_1) \nonumber \\ +&\sum_{h=1}^\infty R(x_2,\pi(x_2))P(X_h = x_2). \label{eq:lem:cIHRSP_IHRSPD:2nd_sum}
\end{align}

Note that because the MDP cannot begin in state $x_2$, $P(X_1 = x_2) = 0$, then the second term in (\ref{eq:lem:cIHRSP_IHRSPD:2nd_sum}) can be index shifted:
\begin{align}
    & \sum_{h=2}^\infty R(X_h = x_2,\pi(x_2))P(X_h = x_2) \\ & = \sum_{h=1}^\infty R(X_{h+1} = x_2,\pi(x_2))P(X_{h+1} = x_2). \label{eq:lem:MIHRSPD_IHRSPD_index_shift}
\end{align}

Additionally, the probability transition law $p_{2,3}(\mathbf{a}) = 1$ guarantees the MDP will only be in state $x_2$ for one epoch immediately after transitioning from state $x_1$. Therefore, $\forall h > h' : P(X_h = x_1 | X_{h'} = x_2) = P(X_h = x_1 | X_{h'} = x_3) = P(X_h = x_2 | X_{h'} = x_2) = P(X_h = x_2 | X_{h'} = x_3) = 0$. So, by the law of total probability we have
\begin{equation}
    P(X_h = x_2) = P(X_h = x_2 | X_{h-1} = x_1)P(X_{h-1} = x_1) \label{eq:lem:MIHRSPD_IHRSPD_total_prob}
\end{equation}

Combining both the index shift (\ref{eq:lem:MIHRSPD_IHRSPD_index_shift}) and total probability (\ref{eq:lem:MIHRSPD_IHRSPD_total_prob}), we can rewrite the final summation to be

\begin{align}
    &E^\pi_x\left[\sum_{h=1}^\infty R(X_h,A_h) \right] = \sum_{h=1}^\infty R(x_1,\pi(x_1))P(X_h = x_1) \nonumber \\ &+ \sum_{h=1}^\infty R(x_2,\pi(x_2)) P(X_{h+1} = x_2 | X_{h} = x_1)P(X_h = x_1)   
    \label{eq:lem:MIHRSPD_IHRSPD_rewritten_final_sum}
\end{align}

One can easily expand the following inner sum found in (\ref{eq:lem:MIHRSPD_IHRSPD_rewritten_final_sum}) using Definitions \ref{def:MIHRSPD_Reward_Functions} and \ref{def:MIHRSPD_P_Transition_Functions} to show that

\begin{align}
    &R(x_1,\pi(x_1)) + R(x_2,\pi(x_2)) P(X_{h+1} = x_2 | X_{h} = x_1) \nonumber \\ &= E(\mathcal{C}_h|\alpha=1)
\end{align}

Using Definition \ref{def:MIHRSPD_P_Transition_Functions}, one can also show that

\begin{align}
    &P(X_{h} = x_1) = P(\alpha_h = 1).
\end{align}

This implies that the expected reward for a given policy $\pi$ (\ref{eq:MIHRSPD_expected_reward}) is equal to the expected reward for its induced package delivery plan $\mathcal{C}$ (\ref{eq:IHRSPD}).
\end{proof}

By an application of Lemma \ref{lem:MIHRSPD_equals_IHRSPD} and the isomorphism between action vectors and package delivery plans, an optimal solution to MIHRSPD will yield an optimal solution to IHRSPD. Using Theorem \ref{thm:stationary_policy}, the optimal package delivery plan must be stationary.


For an instance of IHRSPD, the dispatcher selects a subset of tasks to perform during each epoch. Likewise for a MDP, a controller selects the current action based on some policy during each epoch. To construct the isomorphism between both problems, we will construct a MDP whose action vectors $\mathbf{a} \in A$ are bijective with package delivery plans such that they yield the same expected rewards over an infinite horizon. Specifically, the reward and probability functions of the MDP should have the property that for every unique action vector $\mathbf{a} \in A$, the conditional expected reward for epoch $h$, $E_x^\pi[\sum_{x_i \in S}R(X_h,\mathbf{a})]$, should equal the conditional expected reward (\ref{eq:RSPD_1epoch_expectation}) $E(\mathcal{C}_h | \alpha_h = 1)$ for its ``equivalent'' package delivery plan for epoch $h$ (we will define this properly later). 

We will show that an optimal stationary policy implies a stationary package delivery plan, i.e., $\mathcal{C}_{1} = \mathcal{C}_2 = \ldots $. Under a stationary package delivery plan, the expected reward for an instance of IHRSPD can be solved in $O(n)$ time using the following 
lemma.





Using Lemma \ref{lem:IHRSPD_finite_expected_reward}, if one can construct a MDP $\mathcal{M}$ isomorphic to an instance $\mathcal{I}$ of IHRSPD, then $\mathcal{M}$ will also have a finite expected reward (\ref{eq:MIHRSPD_expected_reward}). Then, if $\mathcal{M}$ satisfies the following theorem, the optimal policy for $\mathcal{M}$ will be stationary and isomorphic to a stationary package delivery plan for $\mathcal{I}$.

==> problem_statement.tex <==
\section{Single Agent Task Allocation}
\subsection{Single Day Case}
Consider an agent that is assigned a set of $n$ tasks $T = \{t_1, t_2, ..., t_n\}$, where each task, $t_i$, has an associated reward, $r_i \in \mathbb{R}_{>0}$. Let $\rho({i,j}) \in [0,1]$ be the probability the agent successfully accomplishes task $t_j$ given its most recent task is $t_i$. The probabilities are symmetric, i.e. $\rho({i,j}) = \rho({j,i})$. We do not consider tasks which can improve the likelihood of success for other tasks, which is equivalent to $\rho({i,j})\rho({j,k}) \leq \rho({i,k})$. This implies their base $\phi \in (0,1)$ logarithms also satisfy the triangle inequality, i.e., $\log_\phi \rho({i,j}) + \log_\phi \rho({j,k}) \geq \log_\phi \rho({i,k})$. If the agent fails, a cost of $\theta$ is incurred and the agent cannot accomplish any future planned tasks.


A walk through $T$ is an ordered, sequence of tasks, $W = \{ t_{w_1}, ..., t_{w_m} \}$, that the agent accomplishes to collect rewards. After the reward from a task is given, the task cannot be accomplished again on the same day. The agent begins in a rest state, represented by a rest task, $t_0$, and can visit the rest task as many times as the agent needs to. The rest task does not give a reward. The agent is limited so it can only accomplish $\mu$ tasks in a row before it must rest. A closed walk is a walk that begins and ends at the same task. Because the agent is limited in the number of tasks it can accomplish before doing the rest task, we can break $W$ into a set of closed walks, $C(W) = \{ W_1, W_2, ..., W_p \}$, each separated by the rest task. Given a closed walk $W = \{ t_{w_1}, t_{w_2}, ..., t_{w_\mu} \}$, let $\psi_{W_i}$ be the probability of accomplishing all tasks in a closed walk, $W_i$, including the previous and last rest task. Then, $\psi_{W_i} = \psi_{W_{i-1}}\rho({0,t_{i,1}})\rho({t_{i,\mu},0})\prod_{j < \mu}{ \rho({t_{i,j},t_{{i,j+1}}})}$. The probability that the agent fails along its walk is equal to the probability it does not finish its last closed walk, i.e. $(1 - \psi_p)$.
 
 Denote $r_{i,m}$ to be the reward of the m-th task in $W_i \in C(W)$, i.e. $t_{i,m} \in W_i$, and let $\psi_{i,m}$ be the probability of receiving reward $r_{i,m}$. For simplicity, we will assume that the reward for all tasks in a cycle are given before beginning of the next cycle, i.e. $\psi_{i,m} < \psi_{j,m'}$ for any $t_{i,m}$ and $t_{j,m'}$ if $i < j$. Then, the reward for a task must be received at some time between accomplishing the task and entering the next rest state. 
 
 We denote the expected reward for a single agent to accomplish its set of ordered walks as:

\begin{equation}
    E(C(W)) = \sum_{i=1}^p\sum_{m=0}^{\mu_i}r_{i,m}\psi_{i,m} - \theta (1 - \psi_p)
\end{equation}

There are two alternative scenarios we consider for when a reward is given. Either the rewards are given upon accomplishing a task, i.e. a package delivery scenario, or they are given during the rest state, i.e. a package collection scenario. The expected reward for each scenario is similar. The properties we prove in this work do not rely on either scenario, however the package delivery scenario maintains the general form. In fact, the package collection scenario can be seen as a restriction on the package delivery scenario by assigning the probability of receiving a task to be the same as the probability of completing the cycle.

\subsection{Package Delivery Scenario}
Impose a maximum number of tasks an agent can accomplish before resting to obtain more packages by an upper limit on the cycles, $\mu_\text{max}$.
\begin{equation}
    E(C(W)) = \sum_{i=1}^p\sum_{m=0}^{\mu_\text{max}}r_{i,m}\psi_{i,m}-\theta(1-\psi_p)
\end{equation}

\subsection{Package Collection Scenario}
By imposing $\forall m \leq \mu_i : \psi_{i,m} = \psi_{i}$, then $\sum_{m=0}^{\mu_i}r_{i,m}\psi_{i,m} = R_i\psi_i$ where $R_i = \sum_{m=0}^{\mu_i}r_{i,m}$.
\begin{equation}
    E(C(W)) = \sum_{i=1}^p R_{i}\psi_{i}-\theta(1-\psi_p)
\end{equation}
This scenario is equivalent to the problem presented in \cite{Prasad_A_2019_Risk_Aware}.

\begin{problem}
 Single-Agent Risk-Aware Task Execution (SARATE)
\end{problem}



==> scrap.tex <==





\begin{equation}
    f(\langle S_\alpha, t_{i,1} \rangle) - f(\langle S_\alpha \rangle) =  r_{t_i} \psi^{d_\alpha +d_i} - \theta(1 - \psi^{d_\alpha +d_i})
\end{equation}

\begin{equation}
    \hat{x_i} = \sum_{y \leq x_i} y P_j(y | x_i) 
\end{equation}

\begin{equation}
    P(j|k) = P(\{ \text{Failed} = k - j\}) 
\end{equation}

Assuming all agents have the same cost, then we can use Poisson trials to calculate the probability of failure. Let $p_\alpha$ be the probability of agent $\alpha$ failing.

\begin{equation}
    P(j|k) = \frac{1}{k + 1}\sum_{n=0}^{k} e^{-\frac{2 \pi i}{k + 1}n(k-j)}\prod_{\alpha=1}^{k} (p_\alpha e^\frac{2 \pi i}{k + 1}+(1 - p_\alpha))
\end{equation}

\begin{equation}
    \hat{x_i} = \frac{1}{x_i + 1}\sum^{x_i,x_i}_{\mu = 0, n = 0}(x_i - \mu)e^{-\frac{2 \pi i}{x_i + 1}} \omega_{x_i}
\end{equation}


Let's assume we generate multi-agent walks by maximizing the reward of an assignment scheme. For example, let $T=\{ t_1, t_2, ..., t_n \}$. We construct the multi-agent walk incrementally by $W_{m + 1} = v(W_{m}, t_j)$ where $t_j = \argmax_{t_i \in T \backslash W_m} E(v(W_{m}, t_i))$. Then, we can define a partial walk on day $i$ as $C_i(W_n)$ where we only take the first $n$ tasks which maximizes the assignment scheme $v(\cdot)$.



\begin{align*}
    & E(k, \hat{n}) = \bar{E}_1(k,n_k) \\ & + \sum_{k_2 = 0}^{k}P_1(k_2 | k)\bar{E}_2(k_2,n_{2,k_2}) + ... \\ &+ \sum_{k_m \leq k_{m-1} \leq ... \leq k} P_m(k_m | k_{m-1})...P_2(k_2 | k)\bar{E}_m(k_m, n_{m,k_m})
\end{align*}

\begin{align*}
    & E(k, \hat{n} \cup \{ n_{m + 1} \}) = \\ & \bar{E}_1(k,n_k) + \sum_{k_2 = 0}^{k}P_1(k_2 | k)\bar{E}_2(k_2,n_{2,k_2}) + ... \\ & + \sum_{k_m \leq ... \leq k} P_m(k_m | k_{m-1})...P_2(k_2 | k)\bar{E}_m(k_m, n_{m,k_m}) \\ & + \sum_{k_{m+1}=0}^k \sum_{t = 0}^{n_{m+1}} \bar{R}_{ {m+1},k_{m+1},t}P_{m+1}(k_{m+1}) \\ & - \theta \sum_{j=0}^{k_{m+1}}(k_{m+1} - j)P_{m+1}(j | k_{m+1})P_{m+1}(k_{m+1})
\end{align*}

\begin{equation}
    P_{m+1}(k_{m+1}) = \sum_{k_m \leq ... \leq k}^{k}P_{m+1}(k_{m+1} | k_m)...P_2(k_2 | k)
\end{equation}

\begin{align*}
    & E_{m+1}(k_{m+1}) = \\ & P_{m+1}(k_m+1)(\sum_{k_{m+1}=0}^k \sum_{t = 0}^{n_{m+1}} \bar{R}_{ {m+1},k_{m+1},t}P_{m+1}(k_{m+1}) \\ & - \theta \sum_{j=0}^{k_{m+1}}(k_{m+1} - j)P_{m+1}(j | k_{m+1})P_{m+1}(k_{m+1})) \\ & = P_{m+1}(k_{m+1})\bar{E}_{m+1}(k_{m+1},n_{m+1})
\end{align*}

\begin{equation}
    E_{m+1}(k) = \sum_{k_{m+1}}^{k}P_{m+1}(k_{m+1})\bar{E}_{m+1}(k_{m+1},n_{m+1})
\end{equation}

\begin{align*}
    = \sum_{k_{m+1} \leq ... \leq k}^{k} & P_{m+1}(k_{m+1} | k_{m})P_{m}(k_{m} | k_{m-1})... \\ & P_2(k_2 | k)\bar{E}_{m+1}(k_{m+1}, n_{{m+1},k_{m+1}})
\end{align*}

\begin{align*}
    E_i(l,n) & =  \sum_{m = 0}^{n}\bar{R}_{i,l,m}P_i(l) - \theta \sum_{j = 0}^l (l-j) P_i(j | l) P_i(l) \\ & = \bar{E}_i(l,n)P(l)
\end{align*}

\begin{align*}
   & V_i(k,m) = \\ & \max_{m'}r_i(k,m) + \theta\sum_{j \leq k}P_{i,m}(j|k)( V_{i+1}(j,m') - \theta(k-j))
\end{align*}

\begin{equation}
    V_n(k,m) = \max_{m'}r_n(k,m) + \sum_{j \leq k}P_{n,m}(j|k)(k-j)
\end{equation}

\begin{align*}
   & V_i(k,m) = \\  \max_{t_m, \bar{m}} & R_i(k, v(W_{i,k,m-1}, t_m)) \\ & + \theta\sum_{l \leq k}P_{i,m}(j|k)( V_{i+1}(l,W_{i+1,l,\bar{m}_l}) - \theta(k-l))
\end{align*}


\subsection{Single Package, Risk-Aware Single Robot Package Delivery (1RSPD)}

\begin{problem}[Single Package, Risk-Aware Single Robot Package Delivery (1RSPD)]
Solve an instance of 1RTPD for $\alpha = 1$. For any instance of 1RSPD, let 
\end{problem}

\begin{corollary}
For 1RSPD, given a  $\psi_p$ be the probability of  the Bellman equation reduces to:
\begin{equation}
    V_h = \max_{\mathcal{C}_{h}} \sum_{W_i \in \mathcal{C}_{h,1}} r_{i}\psi_{i} + \psi_p V_{h+1} - \theta(1 - \psi_p) 
    \label{eq:Bellman_eq_a1_mu1}
\end{equation}

\begin{equation}
    V_k = \sum_{i=1}^p r_{i}\psi_{i}  - \theta(1 - \psi_p) 
    \label{eq:Bellman_eq_base_a1_mu1}
\end{equation}

\end{corollary}

\begin{corollary}
For any instance of 1RSPD, the optimal bound on the reward-to-risk ratio of a cycle reduces to:
\begin{equation}
    \gamma_i > V_{h+1}(\beta) + \theta
\end{equation}
\label{cor:1RTPD_r2r}
\end{corollary}

\begin{equation}
    V_h = \sum_{i=1}^p\sum_{m=0}^{\mu_\text{max}}r_{i,m}\psi_{i,m}-\theta(1-\psi_p) + V_{h+1}  \psi_p
\end{equation}


\begin{lemma}
Consider an instance of 1RSPD with a set of package deliveries, $T = \{ t_1, t_2, ..., t_n \}$, assigned to an agent. If the agent is restricted to one-shot cycles, then taking any delivery whose reward-to-risk ratio satisfies Corollary \ref{cor:1RTPD_r2r} will improve the expected reward. \label{prop:keep_good_r2r}
\end{lemma}

\begin{proof}
We will prove this by contradiction. Suppose it is optimal to take some set of cycles, $\mathcal{C}^*$, which does not include package $t_k$ that satisfies Corollary \ref{cor:1RTPD_r2r}. Let $V_h$ be the Bellman equation for day $h$ when using $T'$:

\begin{equation}
    V_h = \sum_{W_i \in \mathcal{C}^*}\sum_{m=0}^{\mu_\text{max}}r_{i,m}\psi_{i,m} + \psi_p V_{h+1} - \theta(1 - \psi_p) 
\end{equation}

Construct a new set of cycles, $C*$, that includes a task $t_k$ as the last cycle and $\frac{r_k \bar{\psi}_k}{1 - \bar{\psi}_k} > \theta + V_{h+1}$. Note that by Corollary \ref{cor:ordering_of_cycles}, we know the optimal placement of this cycle. So, the overall expected reward can only improve by placing this cycle in the correct spot. However, even this sub-optimal placement is still better than not including it. We denote the new expected reward as:
\begin{equation}
    V^*_h = \sum_{i=1}^p r_{i}\psi_{i} + r_k\bar{\psi}_k\psi_p -\theta(1-\psi_p\bar{\psi}_k) + V_{h+1}\psi_p\bar{\psi}_k
\end{equation}

By assuming $V_h$ is optimal, then $V^*_h - V_h < 0$.

\begin{equation}
    E^*_j - E_j = \psi_p(r_k\bar{\psi}_k - (E_{j+1} + \theta )(1 - \bar{\psi}_k) )  
\end{equation}

But, $\frac{r_k \bar{\psi}_k}{1 - \bar{\psi}_k} > \theta + E_{j+1}$ implies that $E^*_j - E_j > 0$, so $E_j$ is suboptimal.

\end{proof}

\begin{proposition}
Consider an instance of 1RSPD and an ordered set of tasks, $\mathcal{T} = \{ t_1, t_2, ..., t_n \}$, assigned to the agent. The agent visits all tasks in order of reward to risk ratio and the expected reward is denoted $E^*_j$. Suppose we add a new task, $t_k$, to $T$ such that $\frac{r_k \bar{\psi}_k}{1 - \bar{\psi}_k} < \theta + E_{j+1}$ and the new expected reward is $E_j$. Then, $E^*_j > E_j$. I.e. adding a task whose reward to risk ratio is less than $\theta + E_{j+1}$ is always suboptimal.
\end{proposition}

\begin{proof}
We will prove this by contradiction and assume that $E_j$ is optimal. Then, $E_j - E^*_j > 0$. By applying Proposition \ref{prop:keep_good_r2r} and Corollary \ref{cor:ordering_of_cycles}, then $t_k$ must go after all the tasks that satisfy $\frac{r_k \bar{\psi}_k}{1 - \bar{\psi}_k} > \theta + E_{j+1}$. 

\begin{equation}
    E_j - E^*_j = \psi_p(r_k\bar{\psi}_k - (E_{j+1} + \theta )(1 - \bar{\psi}_k) ) + (\psi_k - 1)(\sum_{i=l+1}^p r_{i}\psi_{i})
\end{equation}

However, we know by $\frac{r_k \bar{\psi}_k}{1 - \bar{\psi}_k} < \theta + E_{j+1}$ that the first term must be negative. The second term is always negative because $\psi_k \in [0,1]$. Therefore, $E_j - E^*_j < 0$ which contradicts the optimality of $E_j$.

\end{proof}

\begin{lemma}
    \begin{equation}
        E_h(\mathcal{C}_h|\alpha_h = 1) = \bar{E}(\mathcal{C}_{h})P(\alpha_h = 1)
        \label{eq:expectation_RSPD_epoch_h}
    \end{equation}
    \label{lem:expectation_RSPD_epoch_h}
\end{lemma}
\begin{proof}
To find the total expectation, we sum over all possible rewards and all possible ways of incurring a cost throughout the epoch. Note that $(1 - \bar{\psi}_p)P_h$ is the probability of the agent surviving to epoch $h$ but then failing while following $\mathcal{C}_h$.
$E_h(\mathcal{C}_h)$ is defined explicitly as:
\begin{equation}
        E_h(\mathcal{C}_h) = \sum_{W_i \in \mathcal{C}_h}r_i \bar{\psi}_i P_h - \theta(1 - \bar{\psi}_p)P_h = P_h \bar{E}(\mathcal{C}_{h})
\end{equation}
\end{proof}


\begin{lemma}
Consider an instance of IHRSPD where every package delivery plan is equal, i.e. $\mathcal{C}_{1} = \mathcal{C}_2 = \ldots $. Then, the expected reward for IHRSPD is given by the reward-to-risk ratio of any epoch $\mathcal{C}_{h}$:
\begin{equation}
    \frac{E(\mathcal{C}_{h} | \alpha_1 = 1 )}{1 - \bar{\rho}_{q_h}}
\end{equation}
\end{lemma}
\begin{proof}
Because each package delivery plan is equal $\mathcal{C}_{1} = \mathcal{C}_2 = \ldots$, the expectation for each epoch, Equation (\ref{eq:RSPD_1epoch_expectation}), will also be equal, i.e., $E(\mathcal{C}_{1} | \alpha_1 = 1) = E(\mathcal{C}_{2} | \alpha_2 = 1) = \ldots $. By the same assumption and Equation (\ref{eq:RSPD_q_h}), we can see that $P(\alpha_h = 1) = (\bar{\rho}_{q_h})^{h-1}$. So,

\begin{align}
    \sum_{h = 1}^{\infty} E(\mathcal{C}_{h} | \alpha_h = 1 )&P(\alpha_h = 1) = E(\mathcal{C}_{1} | \alpha_1 = 1 ) \sum_{h = 1}^{\infty} (\bar{\rho}_p)^{(h-1)} \nonumber \\ & = \frac{E(\mathcal{C}_{1} | \alpha_1 = 1 )}{1 - \bar{\rho}_{q_h}} 
\end{align}
\end{proof}

\begin{lemma}
Consider the homogeneous package delivery plan $\mathcal{C}$ for an instance of IHRSPD where $\mathcal{C}_{1} = \mathcal{C}_2 = \ldots $ and the reward-to-risk ratio $\epsilon_1 = \epsilon_2 = ...$ for every epoch is optimal. Swapping any package delivery plan $\mathcal{C}_l \in \mathcal{C}$ with a new package delivery plan $\mathcal{C}^*_{l}$ for epoch $l$ with a lower reward-to-risk ratio will always reduce the expected reward of $\mathcal{C}$. \label{lem:IHRSPD:swap_by_r2r}
\end{lemma}
\begin{proof}
We will prove this by contradiction. Assume $\mathcal{C}^*$ is optimal. Then, using (\ref{eq:IHRSPD}) we have
\begin{align}
    &E(\mathcal{C}^*) - E(\mathcal{C}) = \\ & \sum_{h = 1}^{\infty} E(\mathcal{C}^*_h | \alpha_h = 1 )P(\bar{\alpha}_h = 1) - \sum_{h = 1}^{\infty} E(\mathcal{C}_{h} | \alpha_h = 1 )P(\alpha_h = 1) \nonumber 
\end{align}
Let $\bar{\rho}^*_{l,p} $ and $ \bar{\rho}_{l,q}$ be the probability of the agent surviving package delivery plans $\mathcal{C}^*_l$ and $\mathcal{C}_l$, respectively. Then, by applying (\ref{eq:RSPD_q_h}) we have 
\begin{align}
E&(\mathcal{C}^*) - E(\mathcal{C}) = \\
& [E(\mathcal{C}^*_l | \alpha_h = 1 ) - E(\mathcal{C}_{l} | \alpha_h = 1 )](\prod_{m = 0}^{l-1}\bar{\rho}_{m,p}) \\ &+ (\bar{\rho}^*_{l,p} - \bar{\rho}_{l,q})\sum_{h = l+1}^{\infty} E(\mathcal{C}_h | \alpha_h = 1 )(\prod_{m = l+1}^{h-1}\bar{\rho}_{m,p_m})
\end{align}

Dividing both expressions by $(\prod_{m = 0}^{l-1}\bar{\rho}_{m,p_m})$ yields

\begin{align}
    &\implies [E(\mathcal{C}^*_l | \alpha_h = 1 ) - E(\mathcal{C}_{l} | \alpha_h = 1 )] \\ &+ (\rho^*_{l,p} - \rho_{l,q})\sum_{h = l+1}^{\infty} E(\mathcal{C}_h | \alpha_h = 1 )(\prod_{m = l+1}^{h-1}\bar{\rho}_{m,p_m})
\end{align}
By applying 
\end{proof}

\begin{lemma}
The reward-to-risk ratio $\epsilon_h$ for a package delivery plan $\mathcal{C}_h$ during epoch $h$ is maximal when $\mathcal{C}_h = \{t_{\text{max}}\}$ where $t_{\text{max}}$ is the package delivery with the maximal reward-to-risk ratio, $\epsilon_{\text{max}}$. \label{lem:optimal_package_delivery_horizon}
\end{lemma}
\begin{proof}
We will prove this by contradiction. Let $\mathcal{C}_h = \{t_{\text{max}}\}$ and consider any alternative package delivery plan $\mathcal{C}^*_h$ whose reward-to-risk ratio is greater than $\epsilon_{\text{max}}$. However, $\forall t_i \in \mathcal{C}^*_h : t_i \leq t_\text{max}$ 

\begin{equation}
    \frac{E(\mathcal{C}^*_h | \alpha_h = 1)}{1 - \bar{\rho}_{q_h}} > \frac{E(\mathcal{C}_h | \alpha_h = 1)}{1 - (\rho_1)^2}
\end{equation}

\begin{equation}
    \frac{\sum_i{r_i\psi_i}}{1 - \bar{\rho}_{q_h}} > \frac{r_1 \rho_1}{1 - (\rho_1)^2}
\end{equation}

\begin{equation}
    \sum_i{r_i\psi_i} + r_1\rho_1\bar{\rho}_{q_h} > r_1\rho_1 + \sum_i{r_i\psi_i} (\rho_1)^2 
    \label{lem:eqfinal:optimal_package_delivery_horizon}
\end{equation}

Inequality (\ref{lem:eqfinal:optimal_package_delivery_horizon}) is equivalent to saying the expected reward from a package delivery plan that puts $t_{\text{max}}$ after all packages in $\mathcal{C}^*_h$ is greater than the expected reward for a package delivery plan that puts $t_{\text{max}}$ before $\mathcal{C}^*_h$. However, this contradicts Lemma \ref{lem:ordering_of_cycles} because the reward-to-risk ratio for $t_{\text{max}}$ is greater than or equal to any other package delivery in $\mathcal{C}^*_h$.

\end{proof}

\begin{corollary}
Consider the package with the maximal reward-to-risk ratio, $t_\text{max}$. The optimal package delivery plan for an instance of IHRSPD, $\mathcal{C} = \{ \mathcal{C}_1, \mathcal{C}_2, \ldots \}$ is homogeneous, i.e. $\mathcal{C}_{1} = \mathcal{C}_2 = \ldots $, where $\mathcal{C}_{1} = \{ \{t_\text{max}\}\}$.
\label{cor:optimal_IHRSPD}
\end{corollary}
\begin{proof}
By Lemma \ref{lem:IHRSPD:swap_by_r2r}, swapping out the package delivery plan of any epoch for a package delivery plan with greater reward-to-risk ratio will always improve the expected reward. Therefore, $\mathcal{C}$ is optimal when it is homogeneous with the maximal reward-to-risk ratio for every package delivery plan. Lemma \ref{lem:optimal_package_delivery_horizon} shows that $\mathcal{C}_{1} = \{ \{t_\text{max}\}\}$ has the optimal reward-to-risk ratio of any package delivery plan.
\end{proof}


\begin{lemma}
Consider two possible package delivery plans for epoch $h$, $\mathcal{C}_{h_1}$ and $\mathcal{C}_{h_2}$, where the reward-to-risk ratio for delivery plan $h_1$ is greater than $h_2$, i.e., $\epsilon_{h_1} > \epsilon_{h_2}$. Let $h_p$ and $h_q$ be the index of the last cycles in $\mathcal{C}_{h_1}$ and $\mathcal{C}_{h_2}$, respectively. Then, the following identity holds for any $c \leq \epsilon_1, \epsilon_2$  
\begin{equation}
    E(\mathcal{C}_{h_1} | \alpha_{h} = 1 ) + \bar{\rho}_{h_p} c > E(\mathcal{C}_{h_2} | \alpha_{h} = 1 ) + \bar{\rho}_{h_q} c
    \label{eq:lem:better_R2R_package_delivery}
\end{equation}
\end{lemma}

\begin{proof}
By the assumption $\epsilon_{h_1} > \epsilon_{h_2}$, we have
\begin{equation}
    \frac{E(\mathcal{C}_{h_1} | \alpha_{h} = 1 )}{1 - \bar{\rho}_{h_p}} > \frac{E(\mathcal{C}_{h} | \alpha_{h} = 1 )}{1 - \bar{\rho}_{h_q}} \geq c
\end{equation}

\begin{align}
    \implies E(\mathcal{C}_{h_1} | \alpha_{h} = 1 ) ({1 - \bar{\rho}_{h_q}}) &> E(\mathcal{C}_{h_2} | \alpha_{h} = 1 ) ({1 - \bar{\rho}_{h_p}}) \nonumber \\ & \geq c ({1 - \bar{\rho}_{h_p}})({1 - \bar{\rho}_{h_q}})
\end{align}

\begin{align}
    \implies E(\mathcal{C}_{h_1} | \alpha_{h} = 1 ) &> E(\mathcal{C}_{h_1} | \alpha_{h} = 1 ) ({1 - \bar{\rho}_{h_q}}) \nonumber \\ &> E(\mathcal{C}_{h_2} | \alpha_{h} = 1 ) ({1 - \bar{\rho}_{h_p}}) \nonumber \\ &> c ({1 - \bar{\rho}_{h_p} - \bar{\rho}_{h_q}} + \bar{\rho}_{h_p}\bar{\rho}_{h_q})
    \label{eq:lem:better_R2R_a}
\end{align}

As a necessary aside, consider the following inequality:  
\begin{equation}
    \frac{E(\mathcal{C}_{h_1} | \alpha_{h} = 1 )}{1 - \bar{\rho}_{h_p}} > \frac{E(\mathcal{C}_{h_2} | \alpha_{h} = 1 )}{1 - \bar{\rho}_{h_q}} > E(\mathcal{C}_{h_2} | \alpha_{h} = 1 ) 
\end{equation}


\begin{equation}
    \implies E(\mathcal{C}_{h_1} | \alpha_{h_1} = 1 ) > (1 - \bar{\rho}_{h_p})E(\mathcal{C}_{h_2} | \alpha_{h} = 1 ) \label{eq:lem:better_R2R_b}
\end{equation}

Finally, combine inequalities (\ref{eq:lem:better_R2R_a}) and (\ref{eq:lem:better_R2R_b}).

\begin{align}
    E(\mathcal{C}_{h_1} | \alpha_{h} = 1 ) + c \bar{\rho}_{h_p} &> E(\mathcal{C}_{h_2} | \alpha_{h} = 1 ) + c \bar{\rho}_{2,q} \nonumber \\ &> c (1 + \bar{\rho}_{{h_1},p}\bar{\rho}_{{h_2},q}) > c
\end{align}
\end{proof}

Additionally, if the dispatcher chooses to use the same package delivery plan for every epoch during an instance of IHRSPD, then the infinite sum is equal to the reward-to-risk ratio of the delivery plan.


Due to the equivalence between 

Given that the optimal policy is a stationary policy, we can simplify (\ref{eq:MIHRSPD_expected_reward}) and solve for the optimal policy. Using the law of total probability 

\begin{align}
    E^\pi_x&\left[\sum_{h=0}^\infty R(X_h,A_h) \right] \\ &= \sum_{h=0}^\infty \sum_{i=1}^3 R(X_h = x_i,a^*)P(X_h = x_i) \\ &= \sum_{i=1}^3 \sum_{h=0}^\infty R(X_h = x_i,a^*)P(X_h = x_i) 
\end{align}

\begin{align}
    \sum_{h=0}^\infty &R(X_h = x_1,a^*)P(X_h = x_1) \\ &= R(X_h = x_1,a^*)\sum_{h=0}^\infty(p_{1,1}(a^*))^t = \frac{R(X_h = x_1,a^*)}{1 - p_{1,1}(a^*)}
\end{align}

\begin{align}
    \sum_{h=0}^\infty &R(X_h = x_2,a^*)P(X_h = x_2) \\ &= R(X_h = x_2,a^*)\sum_{h=0}^\infty(p_{1,1}(a^*))^{t-1}(p_{1,2}(a^*)) 
    \\ &= \frac{R(X_h = x_2,a^*)}{p_{1,1}(a^*)}
\end{align}

Because $\forall a \in A(x_3) : R(X_h = x_3,a) = 0$, we have 
\begin{equation}
    \sum_{h=0}^\infty R(X_h = x_3,a^*)P(X_h = x_3) = 0
\end{equation}

Then, 

\begin{align}
    E^\pi_x&\left[\sum_{h=0}^\infty R(X_h,A_h) \right] \\&= \frac{R(X_h = x_1,a^*)}{1 - p_{1,1}(a^*)} + \frac{R(X_h = x_2,a^*)}{p_{1,1}(a^*)} \\ &= \frac{R(X_h = x_1,a^*) - \theta \bar{\psi}(a)}{1 - p_{1,1}(a^*)}
\end{align}

will assume the ansatz stationary policy $\pi(x_0) = \{(1,0,0,...,0)\}$ is optimal. 

